CMB Tensor Anisotropies in f(R) Gravity

The cosmic microwave background (CMB) carries information from the last scattering surface that puts constraints on the multitude of proposed cosmological models and the gravitation theories they are based on. One class of such theories is $f(R)$ gravity, which has become an interesting endeavour to correct for the degeneracies of the concordance model. We presents a description of CMB anisotropies generated by tensor perturbations in $f(R)$ theories of gravity. The temperature and the $E$-mode polarisation power spectra in the special case of $f(R)=R^n$ are computed using a modified version of CAMB package.

==> 0_frontmatter/abbreviations.tex <==
% \chapter*{Abbreviations}
% 
% CMB: Cosmic microwave background\\
% COBE: COsmic Background Explorer\\
% DMR: Differential Microwave Radiometer\\
% FIRAS: Far Infrared Absolute Spectrophotometer\\
% LSS: Large scale structure\\
% SLS: Surface of the last Scattering\\

% \begin{thenomenclature} 
% 
%  \nomgroup{A}
% 
%   \item [{CMB}]\begingroup Cosmic microwave background \nomeqref {0}
% 		\nompageref{viii}
%   \item [{COBE}]\begingroup COsmic Background Explorer \nomeqref {0}
% 		\nompageref{viii}
%   \item [{DMR}]\begingroup Differential Microwave Radiometer\nomeqref {0}
% 		\nompageref{viii}
%   \item [{FIRAS}]\begingroup Far Infrared Absolute Spectrophotometer\nomeqref {0}
% 		\nompageref{viii}
%   \item [{LSS}]\begingroup Large scale structure\nomeqref {0}
% 		\nompageref{viii}
%   \item [{SLS}]\begingroup Surface of the last scattering\nomeqref {0}
% 		\nompageref{viii}
% \end{thenomenclature}

\markboth{{\nomname}}{{\nomname}}
% \markboth{\MakeUppercase{\nomname}}{\MakeUppercase{\nomname}}

% \nomenclature{CMB}{Cosmic Microwave Background}
% \nomenclature{COBE}{COsmic Background Explorer}
% \nomenclature{DMR}{Differential Microwave Radiometer}
% \nomenclature{FIRAS}{Far Infrared Absolute Spectrophotometer}
% \nomenclature{LSS}{Large scale structure}
% \nomenclature{SLS}{Surface of the last scattering}
% \nomenclature{}{}
% \nomenclature{}{}
% \nomenclature{}{}
% \nomenclature{}{}
% \nomenclature{}{}


==> 0_frontmatter/glossary.tex <==
% this file is called up by thesis.tex
% content in this file will be fed into the main document

% Glossary entries are defined with the command \nomenclature{1}{2}
% 1 = Entry name, e.g. abbreviation; 2 = Explanation
% You can place all explanations in this separate file or declare them in the middle of the text. Either way they will be collected in the glossary.

% required to print nomenclature name to page header
\markboth{\MakeUppercase{\nomname}}{\MakeUppercase{\nomname}}


% ----------------------- contents from here ------------------------

% chemicals

\nomenclature{COBE}{COsmic Background Explorer} 

% \nomenclature{DEPC}{diethyl-pyro-carbonate; used to remove RNA-degrading enzymes (RNAases) from water and laboratory utensils}
% \nomenclature{DMSO}{dimethyl sulfoxide; organic solvent, readily passes through skin, cryoprotectant in cell culture}
% \nomenclature{EDTA}{Ethylene-diamine-tetraacetic acid; a chelating (two-pronged) molecule used to sequester most divalent (or trivalent) metal ions, such as calcium (Ca$^{2+}$) and magnesium (Mg$^{2+}$), copper (Cu$^{2+}$), or iron (Fe$^{2+}$ / Fe$^{3+}$)}
% \nomenclature{DAPI}{4',6-diamidino-2-phenylindole; a fluorescent stain that binds strongly to DNA and serves to marks the nucleus in fluorescence microscopy} 




==> 2/cmb.tex <==
% this file is called up by thesis.tex
% content in this file will be fed into the main document

%: ----------------------- name of chapter  -------------------------
\chapter{Covariant Approach to Perturbations in The CMB} % top level followed by section, subsection
\label{cmb}
% 
%: ----------------------- paths to graphics ------------------------
% 
% change according to folder and file names
\ifpdf
    \graphicspath{{X/figures/PNG/}{X/figures/PDF/}{X/figures/}}
\else
    \graphicspath{{X/figures/EPS/}{X/figures/}}
\fi
% 
%: ----------------------- contents from here ------------------------
% 
% 
\section{The Observables}
% 
For every point in space $\vec x$, time $\eta$, and photon incidence direction $\vec e$, the perturbations in the temperature field can be written as:
% 
\begin{equation}
T \l( \vec x,\eta,\vec e \r) = T(\eta) \l[ 1 + \Theta \l( \vec x,\eta,\vec e \r) \r]
\label{tempfield}
\end{equation}
% 
where $\Theta \equiv \frac{\delta T}{T}$. It directly follows that $T \l( \vec x,\eta,\vec e \r) = T(\eta)$ if the copernican principle is assumed. Although $\Theta \l( \vec x,\eta,\vec e \r)$ characterizes $T \l( \vec x,\eta,\vec e \r)$ at every point of spacetime, it can be observed only locally, i.e. at $(\vec x_0, \eta_0)$, given the present means. $\Theta \l( \vec x_0,\eta_0,\vec e \r)$ is stochastic and thus not useful per se. A good statitical tool is the \emph{correlation function}:
% 
\begin{equation}
C(\vartheta) = \la \Theta \l( \vec x_0,\eta_0,\vec e_1 \r) \Theta \l( \vec x_0,\eta_0,\vec e_2 \r) \ra
\label{CF}
\end{equation}
% 
where $\vartheta = \arccos(\vec e_1 \cdot \vec e_2)$ is the relative angle between the photon incidence directions and the angle brackets denote the average over the whole distribution. Expanding the temperature field in terms of spherical harmonics:
%
\begin{equation}
\Theta \l( \vec x_0,\eta_0,\vec e \r) = \sum_{l=1}^\infty \sum_{m=-l}^l a_{lm}(\vec x_0,\eta_0) Y_{lm}(\vec e)
\label{tempsh}
\end{equation}
%

Again, the $a_{lm}$s do not provide any predictions because the randomness of the temperature fluctuations \cite{Dodelson}. The mean of the $a_{lm}$s is zero. the quantity:
%
\begin{equation}
C_l^{TT} = \la a^T_{lm}(\vec x_0,\eta_0) \, a^{* T}_{lm}(\vec x_0,\eta_0) \ra
\end{equation}
%
is the angular power spectrum and measures the variance of the temperature fluctuations at the angular scales corresponding to multipole $l$, approximately $\pi/\vartheta$ \cite{Uzan,Dodelson}.

Using the normalisation of the spherical harmonics:
%
\begin{equation}
\int Y_{lm}(\vec e) Y^*_{lm}(\vec e) d\Omega = 1
\end{equation}
%
and Eq. \eqref{tempsh}, it can be shown that the correlation function in Eq. \eqref{CF} can also be expressed in terms of Legendre Polynomials:
% 
\begin{equation}
C(\vartheta) = \sum_l \frac{2 l + 1}{4 \pi} \Cl \Pl \l( \vec e_1 \cdot \vec e_2 \r)
\end{equation}
% 
The $C_l$s then provide a good characterisation of the CMB at different scales. 

So far, we have only considered the correlation function in temperature. similarly, other observables may be obtained:
%
\begin{equation}
C_l^{X_1X_2} = \la a^{X_1}_{lm}(\vec x_0,\eta_0) \, a^{* X_2}_{lm}(\vec x_0,\eta_0) \ra
\end{equation}
%
where $X_1,X_2 \in \{ T, E, B \}$ \cite{Hu:2002aa,Baskaran:2006qs}. $E$ and $B$ are the E-mode and B-mode polarisations in the CMB.
%
\section{The $1+3$ Formalism}
%
The $1+3$ formalism provides an insightful approach of dealing with the dynamics of cosmological models as it is covariant by construction \cite{Challinor:1999xz}. The following is based on \cite{Ellis:1989jt} \cite{Betschart:2005PhD} \cite[pp 34--35]{Uzan}.
%
\subsection{The Time and Space Projection Tensors}
Spacetime is sliced into constant time hyper-surfaces (rest-space) with respect to fundamental observers with 4-velocity:
%
\begin{equation}
u^a = \frac{dx^a}{d\tau} \qquad \Longrightarrow \qquad u^a u_a = -1
\end{equation}
%
where $\tau$ is the proper time along the observers' world lines. The 4-metric tensor may then be decomposed into time and rest-space symmetric projection tensors:
%
\begin{equation}
g_{ab} = - u_a u_b + h_{ab}
\label{metric_decomp}
\end{equation}
%
The tensor $U_{ab} = - u_a u_b$ projects on the parallel to $u_a$. It can directly be verified that:
%
\begin{equation}
U_{ab} u^a = u_b, \qquad U^a{}_b U^b{}_c = U^a{}_c, \qquad U^a{}_a = 1
\end{equation}
%
while $h_{ab} $ is the rest-space metric tensor. From Eq. \eqref{metric_decomp}, we have:
%
\begin{equation}
h_{ab} u^a = 0, \qquad h^a{}_b h^b{}_c = h^a{}_c, \qquad h^a{}_a = 3
\end{equation}
%
\subsection{Derivatives}
%
Introducing $\epsilon_{abc} \equiv \eta_{abcd}u^d$ is the  projected, totally antisymmetric tensor obtained from $\eta_{abcd}$, the totally antisymmetric tensor on spacetime. Totally antisymmetric tensors of any rank satisfy the identity \cite{Schutz}:
%
\begin{equation}
\epsilon^{ab \ldots c} \, \epsilon_{de \ldots f} = n! \, \delta^a{}_{[d} \, \delta^b{}_e \ldots \delta^c{}_{f]}
\end{equation}
%
where the brackets denote anti-symmetry over the enclosed indices. Hence $\epsilon_{abc}$ satisfies:
%
\begin{subequations}
\begin{eqnarray}
&& \epsilon^{abc} \, \epsilon_{def} = 3! \, h^{[a}{}_d \, h^b{}_e \, \delta^{c]}{}_f\\
&& \epsilon^{abc} \, \epsilon_{cef} = 2! \, h^{[a}{}_e \, h^{b]}{}_f\\
&& \epsilon^{abc} \, \epsilon_{bcf} = 2! \, h^a{}_f \\
&& \epsilon^{abc} \, \epsilon_{abc} = 3!
\end{eqnarray}
\end{subequations}
%

The projected covariant derivative, the time derivative, and the generalized 3-dimensional curl of tensors:
%
\begin{align}
\D_a T_{b\dots}{}^{c\dots} & \equiv h^d_a h^e_b \dots h^c_f \dots \nabla_d T_{e\dots}{}^{f\dots}\\
\dot T_{b\dots}{}^{c\dots} & \equiv  u^a \nabla_a T_{b\dots}{}^{c\dots}\\
\curl T_{ab\dots c} & \equiv \epsilon_{d e (a} \D^d {T_{b\dots c)}}^e
\end{align}
%
where the parentheses denote symmetry over the enclosed indices. $\curl T_{ab\dots c}$ is PSTF for ${T_{ab\dots c}}$ PSTF \cite{Challinor:1999xz}. 
% 
\subsection{Kinematics}
%
Kinematics are obtained by taking the irreducible decomposition of the covariant derivative of the 4-velocity:
%
\begin{equation}
\nabla_a u_b = \frac{1}{3} \Theta h_{ab} + \sigma_{ab} + \omega_{ab} - u_a A_b
\label{velocity_decomp}
\end{equation} 
%
where:
%
\begin{align}
\Theta & \equiv \D^a u_a = 3H \label{expansion_def}\\
\sigma_{ab} =  \sigma_{(ab)} & \equiv\D_{\la a} u_{b \ra} \label{shear_def}\\
\omega_{ab} = \omega_{[ab]} & \equiv \D_{[a}u_{b]} \label{vorticity_def}\\
A_b & \equiv A_b \label{acceleration_def}
\end{align}
%
are the expansion scalar, the shear, the vorticity, and the acceleration, respectively. $H$ is the local Hubble parameter. The angle brackets denote the orthogonal projection of the symmetric trace free part of a tensor and defined as:
%
\begin{equation}
X_{\la ab \ra} \equiv \left[ h_{(a}{}^c \, h_{b)}{}^{d} - \frac{1}{3} \, h_{ab} \, h^{cd} \right] X_{cd}
\label{anglebracket_def}
\end{equation}
%
Another useful kinematic quatity is the projected vorticity vector, defined from the vorticity tensor by:
%
\begin{equation}
\omega_a \equiv \epsilon_{abc} \omega^{bc} /2 = \curl u_a /2
\label{vorticity_vec}
\end{equation}

Deriving directly from equations \eqref{expansion_def}--\eqref{acceleration_def}, we have:
%
\begin{align}
& u^a A_a = 0 \\
& u^a \sigma_{ab} = 0, \qquad \qquad \sigma^a{}_a = 0 \\
& u^a \omega_{ab} = 0, \qquad \qquad \omega^a{}_a = 0
\end{align}
%
which means that the shear and vorticity are PSTF. $A_a$ and $\sigma_{ab}$, and $\omega_a$ characterise anisotropy in the expansion. The projected gradient of the expansion scalar, $\D_a \Theta$, describes inhomogeneity in the expansion. These quantities all vanish in an exact FLRW universe \cite{Challinor:1999xz}.

The last term in the right hand side of Eq. \eqref{velocity_decomp} is the time component of the covariant derivative of the 4-velocity. The definitions in Eq. \eqref{expansion_def}~--~Eq. \eqref{vorticity_def} and Eq. \eqref{anglebracket_def} assert that the shear and expansion terms are the symmetric parts of the rest-space component of $\nabla_a u_b$ while the vorticity term is the antisymmetric part:
%
\begin{equation}
\D_a u_b =  \frac{1}{3} \Theta h_{(ab)} + \sigma_{(ab)} + \omega_{[ab]}
\end{equation}
%
\subsection{Curvature Tensors}
The tidal forces felt by a body moving along a geodesic are represented by the Riemann curvature tensor, $R_{abcd}$, which has the symmetries:
%
\begin{align}
& R_{abcd} = R_{cdab} &&\mathrm{Symmetry\ over\ the\ first\ and\ last\ pair\ of\ indices}\\
& R_{abcd} = R_{[ab][cd]} &&\mathrm{Antisymmetry\ in\ the\ first\ and\ last\ pair\ of\ indices}\\
& R_{a[bcd]} = 0 &&\mathrm{Cyclic\ identity}
\label{Rabcd_sym}
\end{align}
%

The Riemann curvature tensor may be decomposed into its trace and trace-free parts \cite{Ellis:2009go}:
%
\begin{equation}
R_{ab}{}^{cd} = 2 g_{[a}{}^{[c} \, R_{b]}{}^{d]} - \frac{R}{3} \, g_{[a}{}^{[c} \, g_{b]}{}^{d]} + C_{ab}{}^{cd}
\end{equation}
%
where $C_{abcd}$ is the Weyl tensor and describes the vacuum contribution to the gravitational field. It can be decomposed further into a curl-free and a divergence-free PSTF tensors:
 \begin{eqnarray}
E_{ab}  &\equiv&  u^c u^d C_{acbd} \\
H_{ab}  &\equiv&  \frac{1}{2} \, \epsilon_{acd} \, u^e C_{be}{}^{cd}
\end{eqnarray}
%
which are called the \emph{electric} and \emph{magnetic} Weyl tensors, in analogy with the curl-free electric field and divergence-free magnetic field in electromagnetism. $E_{ab}$ is analogous to the tidal tensor derived from the potential in Newtonian gravitation. $H_{ab}$ has no Newtonian counterpart thus is essential for a full description of gravitational waves \cite{Dunsby:1998hd}.
%
\subsection{The Energy-Momentum Tensor}
%
Consider the most general construction of the energy momentum tensor (EMT):
%
\begin{equation}
T_{ab}^{tot} = \rho u_a u_b + p h_{ab} + 2 q_{(a} u_{b)} + \pi_{ab}
\label{EMT}
\end{equation}
%
where $q_a$ and $\pi_{ab}$ are the total energy flux and the total anisotropic stress respectively \cite{Ananda:2007xh}. The following constrains apply:
% 
\begin{equation}
q_a u^a = 0, \qquad \pi_{ab} u^b = 0, \qquad \pi^a{}_a = 0, \qquad \pi_{ab} = \pi_{(ab)}
\label{EMT_constraints}
\end{equation}
% 
The individual components of the EMT can be extracted via the operations:
% 
\begin{subequations}
\label{EMT_decomp_ops}
\begin{align}
\rho &= T_{ab}^{tot} u^a u^b  \\
% \nonumber\\
p &= \frac{1}{3} T_{ab}^{tot} h^{ab} \\
% \nonumber\\
q_a &= -T_{cd}^{tot} u^c h^d{}_a \\
% \nonumber\\
\pi_{ab} &= T_{\la ab \ra}^{tot}
\end{align}    
\end{subequations}
% 
%\subsection{Linearisation}
%
\section{Time Evolution of Perturbations}
%
\subsection{SVT Decomposition}
%
\subsection{Linearisation}
%
 The linearised form is obtained by considering only up to first order (i.e. neglecting $\mathcal{O}(2)$ and higher terms) departures from FLRW \cite{Challinor:1999xz}.

//more on accuracy

\cn
%
\subsection{The Propagation Equations}
%
The evolution of perturbations along the flow lines are described by the propagation equations stated in \cite{Ananda:2007xh,Maartens:1998xg}. Here, we require only the linearised form. There are seven propagation equations:
% 
\begin{eqnarray}
\dot \rho & = & - \l( \rho + p \r) \Theta - \D^a q_a \label{peq1} \\
\dot \Theta & = & - \frac{1}{3} \Theta^2 - \frac{1}{2} \l( \rho + 3p \r) + \D^a A_a \label{peq2} \\
\dot q_a & = & - \frac{4}{3} \Theta q_a - \l( \rho + p \r) A_a - \D_a p - \D^b \pi_{ab} \label{peq3} \\
\dot \omega_a & = & - \frac{2}{3} \Theta \omega_a + \frac{1}{2} \curl A_a \label{peq4} \\
\dot \sigma_{ab} & = & - \frac{2}{3} \Theta \sigma_{ab} - E_{ab} - \frac{1}{2} \pi_{ab} + \D_{\la a} A_{b\ra} \label{peq5}\\
\dot E_{ab} & = & -\Theta E_{ab} + \curl H_{ab} - \frac{1}{2} \l[ (\rho + p)\sigma_{ab} + \D_{\la a} q_{b\ra} + \dot \pi_{ab} + \frac{1}{3} \Theta \pi_{ab} \r] \label{peq6} \\
\dot H_{ab} & = & - \Theta H_{ab} - \curl E_{ab} - {\frac{1}{2}} \curl \pi_{ab}, \label{peq7}
\end{eqnarray}
%
constrained by the following equations:
%
\begin{eqnarray}
\D^a \omega_a  =  0 \label{ceq1}\\
\D^a \sigma_{ab} + \curl \omega_b - {\frac{2}{3}}\D_b \Theta + q_b = 0 \label{ceq2}\\
\D^a E_{ab} +  \frac{1}{3} \Theta q_b - \frac{1}{3} \D_b \rho + \frac{1}{2} \D^a \pi_{ab} = 0 \label{ceq3}\\
\D^a H_{ab} + (\rho + p) \omega_b + \frac{1}{2} \curl q_b = 0 \label{ceq4} \\
H_{ab} - \curl \sigma_{ab} + \D_{\la a} \omega_{b \ra} = 0 \label{ceq5}
\end{eqnarray}
%
The constraints in equations~(\ref{ceq1})--(\ref{ceq5}) are consistent with the linearised propagation equations (\ref{peq1}--\ref{peq7}) \cite{Challinor:1999xz}. //This can be verified by taking the time derivative of a constraint equation. Using the necessary commutation relations and the propagation equations, one should get the constraint equation.

Pure tensor perturbations are obtained by ``turning off'' the scalar and vector modes. This implies that the divergence of the electric and magnetic Weyl tensors together with the vorticity and other projected vectors vanish at first order \cite{Dunsby:1998hd}:
%
\begin{align}
\D^b E_{ab}&=0 \label{tdivE}\\
\D^b H_{ab}&=0 \label{tdivH}
\end{align}
%
\begin{equation}
A_a = 0 \qquad \omega_a = 0 \qquad q_a = 0 \qquad \D_b \rho = 0 \qquad \D_b \Theta = 0 \qquad \ldots
\label{tcond}
\end{equation}
% 
Equations \eqref{tdivE} and \eqref{tdivH} state that the electric and magnetic Weyl tensors are transverse. Indeed, the linearised gravitational waves are described by degrees of freedom of $E_{ab}$ and $H_{ab}$ \cite{Challinor:1999xz}. It is straight forward to verify from Equations \eqref{ceq2} and \eqref{ceq3} that the shear and the anisotropic stress are also divergence free:
\begin{align}
\D^b \sigma_{ab}&=0\\
\D^b \pi_{ab}&=0
\end{align}
%
and that the only constraint that survives is Eq. \eqref{ceq5}. It becomes:
\begin{equation}
H_{ab} = \curl \sigma_{ab}
\label{tceq5}
\end{equation}
The propagation equations~(\ref{peq1})--(\ref{peq7}) reduce to
%
\begin{eqnarray}
\dot \rho &=& -\Theta \l( \rho + p \r) \label{tpeq1}\\
\dot \Theta &=& - \frac{1}{3} \Theta^2 - \frac{1}{2} \l( \rho + 3 p \r) \label{tpeq2}\\
\dot \sigma_{ab} &=& - \frac{2}{3} \, \Theta \, \sigma_{ab} - E_{ab} + \frac{1}{2} \pi_{ab} \label{tpeq3}\\
\dot E_{ab} &=& - E_{ab} \, \Theta + \curl H_{ab} - \frac{1}{2} \l( \rho + p \r) \, \sigma_{ab} - \frac{1}{6} \Theta \, \pi_{ab} - \frac{1}{2} \dot \pi_{ab} \label{tpeq4}\\
\dot H_{ab} &=& - H_{ab}\,\Theta - \curl E_{ab} + \frac{1}{2} \curl \pi_{ab} \label{tpeq5}
\end{eqnarray}
%
Equations \eqref{tpeq3} and \eqref{tceq5} determine the electric and magnetic Weyl tensors, respectively, from the shear.  We now have a closed system of equations. However, Elimination of of the $E_{ab}$ term in Eq. \ref{tpeq3} will require further differentiation.
%
% Making use of the linearised identities~\cite{maartens98}, valid for an arbitrary first-order PSTF tensor $S_{ab}$,
% %
% \begin{eqnarray}
% u^b \nabla_b (\curl S_{ab}) = \curl \dot{S}_{ab} - {\frac{1}{3}}
% \Theta \curl S_{ab} \label{id:1}\\
% u^c \nabla_c (\D^a S_{ab} ) = \D^a \dot{S}_{ab} - {\frac{1}{3}}
% \Theta \D^a S_{ab} \label{id:2} \\
% \D^a (\curl S_{ab}) = {\frac{1}{2}} \curl (\D^a S_{ab}), \label{id:3}
% \end{eqnarray}
% %

\section{Gravitational Waves}
%
Upon the differentiation of equations \eqref{tpeq3}--\eqref{tpeq5} with respect to time, using the energy conservation equation (Eq. \ref{tpeq1}), the Raychaudhuri equation (Eq. \ref{tpeq2}), and the commutator identities (\cn)
\begin{equation}
\curl \dot X_{ab} = (\curl X_{ab})\dot{} + \frac{1}{3} \Theta \curl X_{ab}
\end{equation}
%
\begin{equation}
\curl (\curl S_{ab}) =  \D^2 S_{ab} + {\frac{3K}{S^2}} S_{ab}
- {\frac{3}{2}} \D_{\la a} \D^c S_{b\ra c}.
\label{id:5}
\end{equation}
one arrives to gravitational waves equations for flat models:
%
\begin{align}
\ddot \sigma_{ab} &- \D^2 \sigma_{ab}  + \frac{5}{3} \, \Theta \, \dot \sigma_{ab} + \l( \frac{1}{2} \rho - \frac{3}{2} p 
\r) \, \sigma_{ab} = \dot \pi_{ab} + \frac{2}{3} \, \Theta \, \pi_{ab} \label{gws}\\
\ddot E_{ab} &- \D^2 E_{ab} + \frac{7}{3} \, \Theta \,\dot E_{ab} + \frac{2}{3} \, \l( \rho - p \r) E_{ab}
- \frac{1}{6} \Theta \, \l( \rho + p \r) \, \l( 1 + 3 \, c_s^2 \r) \, \sigma_{ab} \nn\\
&= -\l[ \frac{1}{2} \ddot \pi_{ab} -\frac{1}{2} \D^{2} \pi_{ab} + \frac{5}{6} \, \Theta \, \dot \pi_{ab} + \frac{2}{3}\rho \,\pi_{ab}\r] \label{gwe}\\
\ddot H_{ab} &- \D^2 H_{ab} + \frac{7}{3} \, \Theta \, \dot H_{ab} + 2 \l(\rho - p \r) \, H_{ab}
= \curl \dot \pi_{ab} + \frac{2 }{3} \, \Theta \, \curl \pi_{ab} \label{gwh}
\end{align}

where $c_{s}^{2}=\dot{p}/\dot{\rho}$ and $\D^2 \equiv \D^a \D_a$.  
% 

It can be seen from equations \eqref{gwe} and \eqref{gwh} that the electric and magnetic Weyl tensors play an important role in the propagation of gravitational waves. The curl terms in the corresponding propagation equations gave rise to the wave behaviour in analogy with electromagnetism \cite{Dunsby:1998hd}. Eq. \eqref{gwe} is not closed due to the shear term hence the necessity of deriving the shear wave equation (Eq. \ref{gws}) as well. Moreover, it is more convenient solving for the shear then getting $H_{ab}$ via \eqref{tceq5} rather than starting from Eq. \eqref{gwh}.

\section{Mode Expansion in Tensor Harmonics}
% 
Spacial harmonics are eigenfunctions of the Laplace-Beltrami operator, i.e.:
\begin{equation}
\D^2 Q = - \frac{k^2}{a^2} Q
\label{LBeq}
\end{equation}
%
and are, by construction, covariantly constant:
%
\begin{equation}
\dot Q = 0
\end{equation}
%
where $Q$ represents scalar $\l( Q^{(0)} \r)$, vector $\l( Q^{(1)}_a \r)$, or tensor $\l( Q^{(2)}_{ab} \r)$ harmonics \cite{Bruni:1992dg,Harrison:1967zz}.

Transverse PSTF quantities such as $E_{ab}$, $H_{ab}$, $\sigma_{ab}$, and $\pi_{ab}$ can be expanded in terms of electric and magnetic parity tensor harmonics; $Q_{ab}$ and $\bar Q_{ab}$ respectively \cite{Leong:2002hs}.
%
\begin{subequations}
\begin{align}
E_{ab} &= \sum_{k} \l( \frac{k}{a} \r)^2 \l[ E_k Q_{ab}^{(k)} + \bar E_k \bar Q_{ab}^{(k)} \r] \\ 
H_{ab} &= \sum_{k} \l( \frac{k}{a} \r)^2 \l[ H_k Q_{ab}^{(k)} + \bar H_k \bar Q_{ab}^{(k)} \r] \\ 
\sigma_{ab} &= \sum_{k} \frac{k}{a} \l[ \sigma_k Q_{ab}^{(k)} + \bar \sigma_k \bar Q_{ab}^{(k)} \r] \label{shear_harmonics} \\
\pi_{ab} &= \rho \sum_{k} \l[ \pi_k Q_{ab}^{(k)} + \bar \pi_k \bar Q_{ab}^{(k)} \r]
\end{align}
\label{tensor_harmonics_expansion}
\end{subequations}
%
where $k$ denotes distinct harmonic modes. Tensor harmonic expansion conveniently converts the constraints into algebraic relations and the propagation equations into ordinary differential equations. We have adopted the same expansion as \cite{Challinor:1999xz,Leong:2002hs} for the sake of later comparison.

The electric and magnetic parity tensor harmonics are related via:
%
\begin{subequations}
\begin{eqnarray}
\curl Q^{(k)}_{ab} &=& \frac{k}{a} \, \bar Q^{(k)}_{ab}\\
\curl \bar Q^{(k)}_{ab} &=& \frac{k}{a} \, {Q}^{(k)}_{ab}
\end{eqnarray}
\end{subequations}

These relations reduce Eq. \eqref{tceq5} to:
%
\begin{subequations}
\label{tceq5k}
\begin{eqnarray}
& H_k = \bar \sigma_k \label{tceq5k1} \\ 
& \bar H_k = \sigma_k \label{tceq5k2}    
\end{eqnarray}
\end{subequations}
%

Expanding the shear wave equation (Eq. \ref{gws}) into tensor harmonics using Eq. \eqref{shear_harmonics} and keeping in mind Eq. \eqref{LBeq}, and the Friedmann equations below (Eqs. \ref{friedmann_eqs}), we get:
%
\begin{equation}
\ddot \sigma_k + \Theta \dot \sigma_k + \l[ \frac{k^2}{a^2} - \frac{1}{3} \l( \rho + 3 p \r) \r] \sigma_k = \frac{a}{k} \l[ \rho \dot \pi_k - \frac{1}{3} \l( \rho + 3 p \r) \Theta \pi_k \r]
\label{gwsk}
\end{equation}
%
%// insert the equations for $\ddot E_k$, $\ddot H_k$, and $\ddot \sigma_k$ here.
%
% \begin{subequations}
% \begin{align}
% &\ddot E_k\\
% &\ddot H_k\\

% \end{align}
% \label{wave_equations_k}
% \end{subequations}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Challinor coupled equations %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The constraint equation~(\ref{tceq5}) [or, equivalently,~(\ref{tceq5k})] allows one to eliminate $H_{ab}$
% from the discussion, leaving coupled first-order equations for the
% electric part of the Weyl tensor and the shear:
% %
% \begin{align}
% {\frac{k^2}{S^2}} \left( \dot{E}_k + {\frac{1}{3}} \Theta E_k \right) - {\frac{k}{S}} \left( {\frac{k^2}{S^2}} + {\frac{3K}{S^2}} - {\frac{1}{2}} \gamma \kappa \rho \right) \sigma_k &= - {\frac{1}{6}} (3\gamma - 1) \kappa \rho \Theta \pi_k + {\frac{1}{2}} \kappa\rho \dot{\pi}_k \\
% {\frac{k}{S}} \left(\dot{\sigma}_k + {\frac{1}{3}} \Theta \sigma_k \right) + {\frac{k^2}{S^2}}E_k &= - {\frac{1}{2}} \kappa \rho \pi_k \label{peqh2a}
% \end{align}
% %
% Combining these equations gives the harmonic expansion of the wave equation
% for the shear [equation~(\ref{eq:t2})]:
% %
% \begin{equation}
% \ddot{\sigma}_k + \Theta \dot{\sigma}_k + \left[{\frac{k^2}{S^2}} + {\frac{2K}{S^2}} -{\frac{1}{3}} (3\gamma-2)\kappa \rho \right] \sigma_k = \kappa\rho {\frac{S}{k}} \left[ {\frac{1}{3}} (3\gamma -2) \Theta \pi_k - \dot{\pi}_k \right]. \label{peqh2}
% \end{equation}
% %

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Leong coupled equations %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% 
% Using $H_{ab}={\rm curl}\,\sigma_{ab}$, we arrive at the coupled equations
% 
% \begin{eqnarray} 
% \label{coupled_eqs}
% && \label{Ekprime} \frac{k^2}{a^2} \l(E'_k + \mathcal{H} E_k \r) + k \l[ \frac{1}{2} \l( \rho + p \r) -\frac{k^2}{a^2} \r] \sigma_k = \l[ \rho + \frac{3}{2} p \r] \mathcal{H} \pi_k - \frac{1}{2} \rho \pi'_k \\ 
% && \frac{k}{a^2} \l(\sigma'_k + \mathcal{H} \sigma_k \r) + \frac{k^2}{a^2} E_k = \frac{1}{2} \rho \pi_k 
% \end{eqnarray}
% 
% $\mathcal{H}=a'/a$, and the (non-constant) parameter $\gamma$ is
% defined by $P=(\gamma-1)\rho$. Equations~$\eqref{coupled_eqs}$ and
% $\eqref{Ekprime}$, with all braneworld terms on the right-hand
% sides, determine the tensor anisotropies in the CMB, once $\pi_k$
% is given. The former is determined by the Boltzmann
% equation in the usual way \cite{Challinor:1999xz}, except that the
% background dynamics are altered by braneworld effects. 





% ---------------------------------------------------------------------------
%: ----------------------- end of thesis sub-document ------------------------
% ---------------------------------------------------------------------------



==> 3/fR_theory.tex <==
% this file is called up by thesis.tex
% content in this file will be fed into the main document

%: ----------------------- name of chapter  -------------------------
\chapter{\fR Theories} % top level followed by section, subsection
\label{fR}
% 
%: ----------------------- paths to graphics ------------------------

% change according to folder and file names
\ifpdf
    \graphicspath{{2/figures/PNG/}{2/figures/PDF/}{2/figures/}}
\else
    \graphicspath{{2/figures/EPS/}{2/figures/}}
\fi

%: ----------------------- contents from here ------------------------
% 
% 
\section{The Concordance Model}
%
\subsection{Einstein's Theory of General Relativity}

To model the universe, one needs theories that describe the fundamental interactions. On the large scale, the universe is governed by gravity, the most familiar interaction of them all; yet the least understood. The most successful gravitation theory is Einstein's theory of relativity. It survived many tests at the level of the solar system \cn Uzan?.

\subsubsection{Manifolds}
The metric tensor is one very important, if not the most important, structure defined on a manifold:
%
\begin{equation}
g_{ab} \equiv \vec e_a \cdotp \vec e_b
\label{metric}
\end{equation}
%
where the vectors $\vec e_a$ are the basis of the manifold.

The covariant derivative on the manifold requires the \emph{affine connection} \cite{Clifton:2011jh}:
%
\begin{equation}
\Gamma^a_{\phantom a b c} \equiv  \{^{a}_{\phantom{a} b c}\} + K^a_{\phantom a b c} + L^a_{\phantom a b c}
\label{Gamma} 
\end{equation}
%
where $\{^{a}_{\phantom{a} b c}\}$ is the Levi-Civita connection defined in terms of the metric tensor:
%
\begin{equation}
\{^{a}_{\phantom{a} b c}\} \equiv \frac{1}{2} g^{ad} (g_{bd,c} + g_{cd,b} - g_{bc,d})
\label{LCC} 
\end{equation}
%
$K^a_{\phantom a b c}$ is the contorsion tensor defined in terms of the anti-symmetric parts of the connection:
%
\begin{equation}
K^a_{\phantom a b c} \equiv \Gamma^a_{\phantom a [b c]} - \Gamma^d_{\phantom d [b e]} g^{ae} g_{cd} - \Gamma^d_{\phantom d [c e]} g^{ae} g_{bd}
\label{contorsion} 
\end{equation}
%
or even better in terms of the torsion tensor \cite{ortin2007}:
\begin{equation}
K_{ab}^{\phantom{ab}c} \equiv \frac{1}{2} g^{cd} \l( T_{adb} - T_{bda} - T_{abd} \r) 
\label{contorsion2} 
\end{equation}
%
Finally, $L^a_{\phantom a b c}$ is defined in terms of the non-metricity tensor, $Q_{abc} \equiv \nabla_a g_{bc}$, as:
\begin{equation}
L^a_{\phantom a b c} \equiv \frac{1}{2} \l( Q^a_{\phantom a cb} - Q_{bc}^{\phantom{bc}a} - Q_{cb}^{\phantom{cb}a} \r) 
\label{contorsion2} 
\end{equation}

The GR spacetime is a four dimensional torsionless manifold that satisfies the metric postulate $Q_{abc} = 0$. That is to say that both $K^a_{\phantom a b c}$ and $L^a_{\phantom a b c}$ vanish and the connection, which is now symmetric on the lower indices, reduces to the Levi-Civita connection which is completely defined by the metric tensor.

\subsubsection{The Metric Formalism of GR}

The Einstein-Hilbert in-vacuo Lagrangian $L_{EH}=R$, depending only on the metric tensor and its derivatives (second order at most), is the simplest choice for the gravitational Lagrangian \cite{Hobson}. Here, however, we will include the cosmological constant $\Lambda$ in the gravitational Lagrangian to avoid redundancy:
%
\begin{equation}
L_{GR} = R - 2 \Lambda + L_m(g_{ab},\Psi_m)
\label{GLDE} 
\end{equation}
%
where $L_m(g_{ab},\Psi_m)$ is the contribution the matter field $\Psi_m$ to the gravitational Lagrangian. For convenience, we use the Lagrangian density $\mathcal{L} = L \sqrt{-g}$, where $g$ is the determinant of the metric tensor $g^{ab}$. Varying the action:
%
\begin{equation}
S_{GR} = \int_\mathcal{R} \mathcal{L}_{GR} \ d^4x
\label{actionEHDE} 
\end{equation}
%
with respect to the metric yields to the Einstein field equation (EFE):
% 
\begin{equation}
R_{ab} - \frac{1}{2} \ g_{ab} \ R + \ g_{ab} \ \Lambda = T_{ab}
\label{EFE} 
\end{equation}
% 
where $T_{ab}=-\frac{2}{\sqrt{-g}} \frac{\delta (\mathcal{L}_m)}{\delta g^{ab}}$ \cite{Uzan,Hobson}.

\subsubsection{The Palatini Approach to GR}
An insightful approach to GR
Assume the metric and the connection to be independent fields

one arrives to the fact that indeed the connection is defined in terms of the metric

\subsection{The Cosmological Principle}
%
\emph{The cosmological principle} states that there is no favored location in the Universe. It rises from \emph{isotropy} and the assumption of \emph{homogeneity}. The Universe appears to be isotropic since, at large scales, one starts to see smooth structure in every direction. The CMB has the same temperature over the whole sky to high accuracy; one part in a hundred thousand. Homogeneity, on the other hand, cannot be directly observed. Verifying isotropy in another point in space (2 other points in spherical geometries) \cn would prove homogeneity. Assuming \emph{The Copernican principle} (Earthlings are not privileged observers) implies homogeneity \cn. 


\subsection{FLRW}
The EFE in Eq. \eqref{EFE} is of second order and non linear. A few exact solutions have been produced so far. One of them is the work of Friedmann and Lema\^itre was based on the EFE \cite{Friedmann:1922,Lemaitre:1933gd}. Later, Robertson and Walker \cite{Robertson:1933zz,Walker:1933MNRAS..94..159W} developed a model independently of the EFE by considering the Copernican principle and making use of symmetries. The derivation is covered exhaustively in most, if not all, standard text books. % Proper slicing of spacetime, Proper choice of coordinates
The  The FLRW line element \cite{Hobson}:
% 
\begin{equation}
ds^2 = -dt^2 + a^2(t) d\Sigma^2
\label{FLRWmetric}
\end{equation}
% 
where $dt^2$ and $d\Sigma^2$ are the cosmic time and the spatial intervals. The scale factor $a(t)$ is function of time $t$ and is a measure of the size of the universe. It is normalized to a unit today; i.e. $a(t=\mathrm{now})=1$. In polar coordinates: 
$$d\Sigma^2 = \frac{dr^2}{1+Kr^2} + r^2 \l( d\theta^2 + sin^2\theta \  d\phi^2 \r)$$
where $K\in \{ -1,0,1 \}$ represents open, flat, and closed geometries respectively. It is common to write the FLRW metric in terms of the conformal time, $ d\eta= \frac{dt}{a}$:
% 
\begin{equation}
ds^2 = a^2(\eta) \l[ -d\eta^2 + \frac{dr^2}{1+Kr^2} + r^2 \l( d\theta^2 + sin^2\theta \  d\phi^2 \r) \r]
\end{equation}
% 

Using the FLRW metric, an alternate form of the EFE
%
\begin{equation}
R_{ab} = T_{ab} + \frac{1}{2} \ g_{ab} \ R + \ g_{ab} \ \Lambda
\label{EFEalternate} 
\end{equation}
%
and the perfect fluid model for the EMT,
%
\begin{equation}
T_{ab} = (\rho -p) u_a u_b + p g_{ab},
\label{EMTperfect} 
\end{equation}
%
one gets the cosmological field equations; also known as the Friedmann--Lema\^itre equations \cite{Hobson}:
%
\begin{subequations}
\label{friedmann_eqs}
\begin{eqnarray} 
&& H^2 = \frac{1}{3} \rho + \frac{1}{3} \Lambda - K \label{friedmann_dot}\\
&& \frac{\ddot a}{a} = - \frac{1}{6} \l(\rho + 3 p \r) + \frac{1}{3} \Lambda \label{friedmann_ddot}
\end{eqnarray}
\end{subequations}
%
where the dot denotes the differentiation with respect the the cosmic time $t$. 

On the other hand, the energy conservation condition, $\nabla^a T_{ab}$ leads to the equation of motion (EoM) of the cosmological fluid:
\begin{equation}
\dot \rho + 3 H \l( \rho + p \r) =0
\label{Econserv}
\end{equation}
%
Only two of Equations \eqref{friedmann_dot}, \eqref{friedmann_ddot}, and \eqref{Econserv} are independent. The third is inferred easily.

To close the system, a relation between the pressure and the density of the fluid $p=p(\rho)$ is needed. The equation of state (EoS) $\omega$ of the fluid plays just this role: 
%
\begin{equation}
p = \omega \rho
\label{EoS}
\end{equation}
%
$\omega$ is usually constant in time except for some cosmologies which require $\omega=\omega(t)$ \cite{Hobson}. 


\subsection{The Concordance Model}
%
The universe we live in is not as smooth as an FLRW universe would be; but rather \emph{perturbed}. $\Lambda$CDM, is the best fit model to observations cosmologists have. To achieve this status, 95\% of the content of the universe had to be \emph{dark} \cite{Clifton:2011jh}. Indeed, $\Lambda$CDM claims that observable baryonic matter constitutes only 4 to 5\% of the total energy density of the universe. Another 25\% is in the form of non-relativistic \emph{dark matter} interacting only gravitationally. Dark matter was strongly suggested by rotational curves of disk galaxies \cite{Rubin:1985ze}. The surprising discovery of the acceleration of the expansion of the universe through distant type Ia supernovae measurement \cite{Perlmutter:1997zf,Riess:1998cb,Perlmutter:1998np} imposed that the remaining 70\% of the energy density in the $\Lambda$CDM picture picture has to be some unknown form of energy with anti-gravitational properties. This became known as \emph{dark energy}.
%
\subsection{Beyond The Standard Model}
The concordance model suffers from a few problems (Cusp-core problem \cite{deBlok:2009sp,Li:2009mp}, missing satellite problem \cite{Bullock:2010uy} \ldots etc) out of which that of the cosmological constant is the most severe \cite{Clifton:2011jh}. The energy density $\rho_\Lambda$ calculated at near the Planck scales value is 120 orders of magnitude larger than the upper bound set by cosmological observations. Proposed mechanisms (such as super-symmetry theories) to reconcile these results have to be accurate to within 120 decimal places causing a \emph{fine tuning problem}. In addition, the current densities of matter and vacuum energy are of of the same order of magnitude, $\rho_{\Lambda,0} \approx \rho_{m,0}$. This is the so called \emph{coincidence problem} \cite{Weinberg:2000yb,Clifton:2011jh}.

The problems with the $\Lambda$CDM model mainly reflect the shortcomings of the classical theory of general relativity. This created the need/opportunity to investigate more general theories of gravity. The idea is almost as old as GR itself. Barely a few years after Einstein published his paper (\cite{Einstein:1915by}), there were already suggestions of modifying the Einstein-Hilbert action by introducing higher order terms \cite{Weyl:1919fi,Eddington1923}. The first requirement of any gravitation theory is the crucial condition of fitting astrophysical and cosmological observations. \emph{extended theories of gravity} strive to build up on the success of GR by introducing corrections either through coupling geometry to a scalar field in which case the result is a scalar-tensor theory of gravity, or by adding higher order curvature invariants to the gravitational Lagrangian; this accordingly yields to higher order field equations \cite{Capozziello:2007ec}. So while attempting to explain the universe at high regimes, ETGs should absolutely reduce to GR in the weak field limit.

//Quantization of gravity.

% //assume the Copernican principle to retain an FLRW universe \cite{Clarkson:2010uz,Stoeger:1994qs}
% 
\section{Overview of \fR Gravity}

\fR theories of gravity, first studied in \cite{Buchdahl:1983zz}, are a class of ETGs and represent one of the simplest modification to GR. They arise from replacing the Ricci scalar $R$ in the Einstein-Hilbert Lagrangian with a more general and arbitrary function \fR  \cite{Sotiriou:2008rp,DeFelice:2010aj}. While the metric and Palatini formalisms of the theory of general relativity lead to the same field equation due to the linearity of the Lagrangian in $R$, one would not expect the same for higher order theories of gravity \cite{Capozziello:2009nq}. Indeed, there are three formalism of \fR concisely presented below. For a more extensive description, the reader is referred to \cite{Sotiriou:2007yd}. 

\subsection{The Metric Formalism}
% [It is also possible to show that \fR gravity is equivalent not only to a scalar-tensor theory, but also to GR plus an ideal fluid](verbatim from \cite{Capozziello:2009nq})
Variation with respect to the metric of the \fR action:
\begin{equation}
    \label{actionfR} 
    S_{metric} = \int_\mathcal{R} f(R) \sqrt{-g} + \mathcal{L}_m(g_{ab},\Psi_m) \ d^4x
\end{equation}
%
leads to a fourth order gravitational field equation:

\begin{equation}
R_{ab} - \frac{1}{2} \ g_{ab} \ R  = \frac{1}{f_R} \ T_{ab} +  \frac{1}{f_R} \l[ \frac{1}{2} \ g_{ab} \ f + \l(\nabla_a \nabla_b - g_{ab} \Box \r) f_R  - \frac{1}{2} \ f_R \ g_{ab} \ R \r]
\label{FE}
\end{equation}

\noindent where $f_R \equiv \frac{df}{dR}$. 
\subsection{The Palatini Formalism}
\subsection{The Metric-affine Formalism}

\cite{Capozziello:2009nq}

\subsection{The Cosmological Field equations in \fR}
The Friedmann Equations in \fR, maintain the same form as in Equations \eqref{friedmann_eqs}. In conformal time, they read:

\begin{subequations}
\label{friedmann_eqs_tau}
\begin{eqnarray} 
&& \mathcal{H}^2 = \frac{1}{3} \rho a^2 \\
&& \mathcal{H} ' = - \frac{a^2}{6} \l(\rho + 3 p \r) \\
&& \rho' + 3 \mathcal{H} \l( \rho + p \r) =0
\end{eqnarray}
\end{subequations}
%
where the prime is the differentiation with respect to the conformal time $\eta$ and $\mathcal{H} = \frac{a'}{a}$. The higher order geometric information of \fR is encoded in the scale factor $a(t$), the density $\rho$, and the pressure $p$.


%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%
\section{The Dynamics of \fR Cosmologies}
%
The field equation in Eq. \eqref{FE} is written in such way to keep the traditional Einstein tensor on the left hand side. The first term of the right hand side may be interpreted as the effective contribution of standard matter in the new geometry. The second term is fully geometric and will be referred, hereafter, as the \emph{curvature fluid}. This multi-fluid decomposition is useful in the sense that the covariant approach can be applied the usual way once the thermodynamics of the fluids have been determined \cite{Ananda:2007xh}.
%

Applying the operations in Equations \ref{EMT_decomp_ops} to the EMT, We get:
% 
\begin{subequations}
\label{EMT_decomp}
\begin{align}
\rho &= \frac{\rho^m}{f_R} + \rho^R \\
% \nonumber\\
p &= \frac{p^m}{f_R} + p^R \\
% \nonumber\\
q_a &= \frac{q_{a}^m}{f_R} + q_{a}^R \\
% \nonumber\\
\pi_{ab} &= \frac{\pi_{ab}^m}{f_R} + \pi_{ab}^R \label{anis_decomp}
\end{align}
\end{subequations}
%
where the superscript ``$^R$'' indicates the contribution of the curvature fluid to the components of the EMT. The linearised components of the curvature fluid are found to be: 
%
\begin{subequations}
\label{curvature_fluid}
\begin{align}
\rho^{R} &= \frac{1}{f_R} \l[ \frac{1}{2}(R f_R-f)-\Theta f_{2R}\dot{R}+f_{2R}\tilde{\nabla}^2{R} \r] \\
p^{R} &= \frac{1}{f_R} \l[ \frac{1}{2}(f-Rf_R)+f_{2R}\ddot{R}+f_{3R}\dot{R}^2+\frac{2}{3}\Theta f_{2R}\dot{R} -\frac{2}{3}f_{2R}\tilde{\nabla}^2{R} \r] \\
q^{R}_a &= \frac{1}{f_R} \l[ - f_{3R}\dot{R}\D_{a}R - f_{2R}\D_{a}\dot{R} + \frac{1}{3}f_{2R} \D_{a}R \r] \\
\pi^{R}_{ab} &= \frac{1}{f_R} \l[ f_{2R}\D_{\lgl a}\D_{b\rgl}R - f_{2R} \, \sigma_{ab}\dot{R} \r] \label{curvature_anis}
\end{align}
\end{subequations}
%
which reduce, in pure tensor modes, to:
%
\begin{equation}
\pi^{R}_{ab} = - \frac{f_{2R}}{f_R} \, \sigma_{ab}\dot{R}  
\label{curvature_anis}
\end{equation}



% \section{Data}
% 
% \begin{table}[htdp]
% \centering
% \begin{tabular}{|l|c|c|l|c|} % l|l|l|
% \hline
% {\bf Object} & \multicolumn{2}{|l|}{{\bf Coordinates (J2000)}}  & {\bf Redshift} & {\bf Distance (Mpc)} \\
% \cline{2-3}
% &$\alpha$&$\delta$&&\\
% \hline
% IRAS 05368+4940 & 05 40 43.71 & +49 41 41.5 & 0.019157 & 79.9 \\% & & & \\
% \hline
% IC 694 & 11 28 27.30 & +58 34 42.5 & 0.013200 & 57 \\%& 9.628 & 9.847 & 8.422 \\
% \hline
% IRAS 11257+5850 & 11 28 32.20 & +58 33 44.0 & 0.010411 & 45.3 \\%& & & \\
% 
% \hline
% 
% \end{tabular}
% \caption[The Galaxy Sample]{\textbf{The Galaxy Sample.} (from  \href{http://nedwww.ipac.caltech.edu/indexFrames.html}{NASA/IPAC extragalactic Database.})}
% \label{sample}
% \end{table}
% 
% 
% 
% \begin{center}
% \begin{longtable}[htdp]{|l|c|c|c|c|c|c|} 
% \hline
% {\bf Object} & {\bf m}  & {\bf M} & {\bf Re (pix)} & {\bf Re (kpc)} & {\bf b/a} & {\bf D/B} \\
% \hline
% IRAS 05368+4940: & & & & & & \\
% exp & 9.79 & -24.72 & 48.31 & 0.42 & 0.6 & -0.26 \\
% devauc & 13.93 & -20.58 & 34.75 & 0.30 & 0.3 & -1.18 \\
% \hline
% IC 694: & & & & & & \\
% exp & 9.74 & -24.04 & 13.63 & 0.19 & 0.8 & -0.11 \\
% devauc & 12.03 & -21.75 & 99.31 & 0.60 & 1.0 & -0.8 \\
% \hline
% 
% \caption[Exponential Disk and De Vaucouleurs Profiles of Gemini/Altair and VLT/NaCo data]{\textbf{Exponential Disk and De Vaucouleurs Profiles for Gemini and VLT Images} - m and M are the apparent and absolute magnitudes respectively, Re is the effective radius, b/a is the axis ratio, D/B is the diskiness (negative) and boxiness (positive) of the isophotes.}
% \label{expdevauc}
% \end{longtable}
% \end{center}



% ---------------------------------------------------------------------------
%: ----------------------- end of thesis sub-document ------------------------
% ---------------------------------------------------------------------------



==> 4/anis_fR.tex <==
% this file is called up by thesis.tex
% content in this file will be fed into the main document

%: ----------------------- name of chapter  -------------------------
\chapter{CMB Tensor Anisotropies in \fR Gravity} % top level followed by section, subsection
\label{anis_fR}


%: ----------------------- paths to graphics ------------------------

% change according to folder and file names
\ifpdf
    \graphicspath{{X/figures/PNG/}{X/figures/PDF/}{X/figures/}}
\else
    \graphicspath{{X/figures/EPS/}{X/figures/}}
\fi

%: ----------------------- contents from here ------------------------


\section{The Wave Equation}
In the radiation dominated era: $\pi^m=\pi^\gamma$. //turn off scalar and vector modes. 
using Equations \ref{anis_decomp} and \ref{curvature_anis}, Eq. \eqref{gwsk} becomes, to first order:
\begin{equation}
\ddot \sigma_k + A \dot \sigma_k + B \sigma_k = \frac{a}{k} \frac{\rho}{f_R} \l[ \dot \pi^\gamma_k - \l( H + 3H\omega +
\frac{f_{2R}}{f_R} \r) \pi^\gamma_k \r] 
\label{shear_wave_eq_k}
\end{equation}
with $$A = 3H + \frac{f_{2R}}{f_R} \dot R$$ and $$B = \frac{k^2}{a^2} + 2 \frac{\ddot a}{a} + \dot R^2 \l( \frac{f_{3R}}{f_R} -\l( \frac{f_{2R}}{f_R} \r) ^2 \r) + \frac{f_{2R}}{f_R} \ddot R + H \frac{f_{2R}}{f_R} \dot R $$



Neglecting the radiation anisotropic stress and changing to conformal time, Eq. \eqref{shear_wave_eq_k} becomes:

\begin{equation}
\sigma_k '' + \l( a A - \mathcal{H} \r) \sigma_k ' + a^2 B \sigma_k =  0
\label{shear_wave_eq_eta}
\end{equation}

Making the variable change $u_k = a^m \sigma_k$ and choosing $m = \frac{Aa - \mathcal{H}}{2 \mathcal{H}}$, Eq.
(\ref{shear_wave_eq_eta}) becomes:

\begin{equation}
u_k '' + \l[ - \frac{1}{2} m \mathcal{H} \frac{f_{2R}}{f_R} R' - m \frac{a''}{a} + a^2 B \r] u_k = 0
\label{uwave}
\end{equation}


\section{The Case of $f(R) = R^n$}


For the case of $f(R) = R^n$, \cn
$$R = 6 \frac{a''}{a^3}$$
\cn

Introducing the parameter \hspace{0.5cm} $\varepsilon \equiv \frac{2n}{3(1 + \omega)} -1 $ \hspace{0.5cm} such that \hspace{0.5cm} $a(\eta) = \eta^{-\frac{1+\varepsilon}{\varepsilon}}$

m becomes $$m = 1 + \frac{1-n}{1+\varepsilon}$$
and Eq.(\ref{uwave})

the equation of motion
\begin{equation}
u_k'' + \l[k^2 + m \l( \frac{\varepsilon + 1}{\varepsilon^2} \r) \l( n-2 \r) \eta^{-2} \r] u_k = u_k'' + \l[k^2 - \frac{(a^{-m})''}{a^{-m}} \r] u_k = 0
\label{EoM}
\end{equation}

We are dealing here with the initial conditions of the perturbations which means we are deep in the radiation dominated era. The equation of state is thus $\omega=\frac{1}{3}$. Eq.\eqref{EoM} becomes:

\begin{equation}
u_k'' + \l[k^2 - 2 \eta^{-2} \r] u_k = 0
\end{equation}

 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% 
% 
% 
% 
% ///////////////////////////////////////////////////////////////
% 
% In flat models ($K=0$)
% on large scales there is a decaying solution $\sigma_k \propto
% a^{-2m} $. Since Eq. contains no first
% derivative term the Wronskian is conserved. On large scales we can
% use the solution $\sigma_k \propto a^{-2m} $ to write the
% conserved Wronskian as $W = \sigma_k' + 2m\mathcal{H} \sigma_k
% $. (The Wronskian vanishes in the decaying mode.) Integrating
% gives the following two independent solutions on large scales in
% flat models:
% \begin{equation}
% \sigma_k=
% \begin{cases}
% A_k a^{-2m} \,,\\ B_k a^{-2m} \int^{\tau}
% d\tilde\tau\, a(\tilde\tau)^{2m} \, ,
% \end{cases}
% \end{equation}
% where $A_k$ and $B_k$ are constants of integration. If we let
% $\zeta \to 0$, we recover the results in \cite{Lewis:2000PhD} for
% the general relativity case.
% 
% The conserved Wronskian is proportional to the metric perturbation
% variable, $H_T$, characterising the amplitude of 4D gravitational
% waves. In flat models $H_T$ is related to the covariant variables
% quite generally by
% \begin{equation} \label{e:HT1}
% H_{Tk} = \frac{\sigma'_k}{k} + 2 E_k \, .
% \end{equation}
% Ignoring photon anisotropic stress, we can eliminate the electric
% part of the Weyl tensor via the shear propagation
% equation~(\ref{coupled_eqs}) to find $k H_{Tk} = - \sigma_k' -
% (\zeta + 2) \mathcal{H} \sigma_k = -W$. The fact that $H_T$ is
% conserved on large scales in flat models in the absence of photon
% anisotropic stress can also be seen directly from its propagation
% equation,
% \begin{equation}
% H_{Tk}'' + 2m \mathcal{H} H_{Tk}' + k^2 H_{Tk} = 0\,.
% \end{equation}
% 
% We can solve Eq.~(\ref{uwave}) on all scales in the high-energy
% ($\rho\gg \lambda$ and $a\propto \tau^{1/3}$) and low-energy
% ($\rho\ll\lambda$ and $a\propto \tau$) radiation-dominated
% regimes, and during matter-domination ($a\propto \tau^2$). The
% solutions are
% \begin{align}
% \label{e:highenergy1} u_k(\tau) &= \sqrt{k\tau} \left[ c_1
% J_{\frac{1}{6}(2m + 3)} (k \tau)  + c_2 Y_{\frac{1}{6}(2m + 3)}
% (k \tau)\right] & \quad &(\text{high energy radiation}), \\
% \label{e:lowenergy1} u_k(\tau) &= \sqrt{k\tau} \left[c_3
% J_{\frac{1}{2} (2m + 1)} (k \tau) + c_4 Y_{\frac{1}{2}(2m + 1)}
% (k \tau)\right] & &(\text{low energy radiation}),\\
% \label{e:matter} u_k(\tau) &= \sqrt{k\tau} \left[ c_5
% J_{2m - \frac{1}{2}} (k \tau)  + c_6 Y_{2m - \frac{1}{2}} (k
% \tau)\right] & &(\text{matter domination}),
% \end{align}
% where $c_i$ are integration constants. The solutions for the
% electric part of the Weyl tensor can be found from
% Eq.~(\ref{coupled_eqs}). For modes of cosmological interest the
% wavelength is well outside the Hubble radius at the transition
% from the high-energy regime to the low-energy. It follows that the
% regular solution (labelled by $c_1$) in the high-energy regime
% will only excite the regular solution ($c_3$) in the low-energy,
% radiation-dominated era. Performing a series expansion, we arrive
% at the appropriate initial conditions for large-scale modes in the
% low-energy radiation era:
% \begin{align}
% H_{Tk} &=  1 - \frac{(k \tau)^2}{2 (3 + \zeta)} + \frac{(k \tau)^4}{8 (2m + 1)(2m + 3)}  + O[(k\tau)^6] \label{e:hijini} \\
% \sigma_k &= -\frac{k \tau}{2m + 1} + \frac{k^3 \tau^3}{2(2m + 1)(2m + 3)} + O[(k\tau)^5] \label{e:shearini}\\
% E_k &=  \frac{m + 1}{2m + 1} - \frac{(k\tau)^2 (m+3)}{2(2m + 1)(2m+3)} + O[(k\tau)^4] \label{e:elecini} 
% \end{align}
% In the limit $\zeta \to 0$, we recover the general relativity
% results in \cite{Challinor:1999zj}.
% 
% For modes that are super-Hubble at matter-radiation equality
% (i.e.\ $k \tau_{\text{eq}} \ll 1$), the above solution joins
% smoothly onto the regular solution labelled by $c_5$ in
% Eq.~(\ref{e:matter}). For $k \tau_{\text{eq}} \gg 1$, the shear
% during matter domination takes the form
% \begin{equation}
% \label{e:matterlong} 
% \sigma_k = - 2^{2m - \frac{1}{2}}\Gamma \l( 2m + \frac{1}{2} \r) (k\tau)^{- \l( 2m - \frac{1}{2} \r) } J_{2m - \frac{1}{2}}(k\tau).
% \end{equation}
% In the opposite limit, the wavelength is well inside the Hubble
% radius at matter-radiation equality. The asymptotic form of the
% shear in matter domination is then
% \begin{equation}
% \label{e:mattershort} 
% \sigma_k \sim \frac{\Gamma \l( m + \frac{1}{2} \r)}{\sqrt{\pi}} \left( \frac{2 \, \tau_{\text{eq}}}{\tau}\right)^m (k\tau)^{-m} \sin \l( k\tau - \pi \frac{m-1}{2} \r)
% \end{equation}
% 


\section{CAMB}
camb, code for anisotropies in the microwave backgoung, is  a fortran package wriiten by antony lewis and the guy before him based on cmb easy by seljak and zaldarriaga. 
lewis converted it to f90 , Camb described in \cite{Lewis:2000PhD}.
We modified the code for the case of the brane already investigated by leong et al. (2002) and we reproduced their results. We then set out to modify Camb for $f(R)=R^n$. This proved to be difficult because of the huge difference in the background. We provide a fitting functions of $H^2$ from which we define other quantities such as $\frac{da}{d\eta}$.
the results are discussed below.

\section{Power Spectra}



% ---------------------------------------------------------------------------
%: ----------------------- end of thesis sub-document ------------------------
% ---------------------------------------------------------------------------



==> 5/discussion.tex <==
% this file is called up by thesis.tex
% content in this file will be fed into the main document

%: ----------------------- name of chapter  -------------------------
\chapter{Discussion and Conclusions} % top level followed by section, subsection
\label{discussion}


%: ----------------------- paths to graphics ------------------------

% change according to folder and file names
\ifpdf
    \graphicspath{{X/figures/PNG/}{X/figures/PDF/}{X/figures/}}
\else
    \graphicspath{{X/figures/EPS/}{X/figures/}}
\fi

%: ----------------------- contents from here ------------------------

\section{Discussion}
Results\\
Comparison with previous work BW and GR
\section{Neglected Corrections}
No neutrinos\\
No secondary anisotropies, reionization effects\\
\ldots

\section{Future Work}


% ---------------------------------------------------------------------------
%: ----------------------- end of thesis sub-document ------------------------
% ---------------------------------------------------------------------------



==> 6/perturbations.tex <==
% this file is called up by thesis.tex
% content in this file will be fed into the main document

%: ----------------------- name of chapter  -------------------------
\chapter{Perturbation Equations in $f(R)$ Gravity} % top level followed by section, subsection
\label{perturbations}

%: ----------------------- paths to graphics ------------------------

% change according to folder and file names
\ifpdf
    \graphicspath{{3/figures/PNG/}{3/figures/PDF/}{3/figures/}}
\else
    \graphicspath{{3/figures/EPS/}{3/figures/}}
\fi

%: ----------------------- contents from here ------------------------





% ---------------------------------------------------------------------------
%: ----------------------- end of thesis sub-document ------------------------
% ---------------------------------------------------------------------------



==> 7/citetest.tex <==
\chapter{2}
\cite{Leong:2002hs}


==> 7/materials_methods.tex <==

% this file is called up by thesis.tex
% content in this file will be fed into the main document

\chapter{Materials \& methods} % top level followed by section, subsection


% ----------------------- paths to graphics ------------------------

% change according to folder and file names
\ifpdf
    \graphicspath{{8/figures/PNG/}{8/figures/PDF/}{8/figures/}}
\else
    \graphicspath{{8/figures/EPS/}{8/figures/}}
\fi

% ----------------------- contents from here ------------------------




 

% ---------------------------------------------------------------------------
%: ----------------------- end of thesis sub-document ------------------------
% ---------------------------------------------------------------------------



 








==> 8/1+3.tex <==
% this file is called up by thesis.tex
% content in this file will be fed into the main document

\chapter{The $1+3$ Formalism of Perturbations in Cosmology} % top level followed by section, subsection
\label{1+3}

% ----------------------- paths to graphics ------------------------

% change according to folder and file names
\ifpdf
    \graphicspath{{7/figures/PNG/}{7/figures/PDF/}{7/figures/}}
\else
    \graphicspath{{7/figures/EPS/}{7/figures/}}
\fi


% ----------------------- contents from here ------------------------

The $1+3$ formalism provides an insightful approach of dealing with the dynamics of cosmological models as it is covariant by construction \cite{Challinor:1999xz}. The following is based on \cite{Ellis:1989jt} \cite{Betschart:2005PhD} \cite[pp 34--35]{Uzan}.
Spacetime is sliced into constant time hyper-surfaces (rest-space) with respect to fundamental observers with 4-velocity:
%
\begin{equation}
u^a = \frac{dx^a}{d\tau} \qquad \Longrightarrow \qquad u^a u_a = -1
\end{equation}
%
where $\tau$ is the proper time along the observers' world lines. The 4-metric tensor may then be decomposed into time and rest-space symmetric projection tensors:
%
\begin{equation}
g_{ab} = - u_a u_b + h_{ab}
\label{metric_decomp}
\end{equation}
%
The tensor $U_{ab} = - u_a u_b$ projects on the parallel to $u_a$. It can directly be verified that:
%
\begin{equation}
U_{ab} u^a = u_b, \qquad U^a{}_b U^b{}_c = U^a{}_c, \qquad U^a{}_a = 1
\end{equation}
%
while $h_{ab} $ is the rest-space metric tensor. From Eq. \eqref{metric_decomp}, we have:
%
\begin{equation}
h_{ab} u^a = 0, \qquad h^a{}_b h^b{}_c = h^a{}_c, \qquad h^a{}_a = 3
\end{equation}

Introducing $\epsilon_{abc} \equiv \eta_{abcd}u^d$ is the  projected, totally antisymmetric tensor obtained from $\eta_{abcd}$, the totally antisymmetric tensor on spacetime. Totally antisymmetric tensors of any rank satisfy the identity \cite{Schutz}:
%
\begin{equation}
\epsilon^{ab \ldots c} \, \epsilon_{de \ldots f} = n! \, \delta^a{}_{[d} \, \delta^b{}_e \ldots \delta^c{}_{f]}
\end{equation}
%
hence $\epsilon_{abc}$ satisfies:
%
\begin{subequations}
\begin{eqnarray}
&& \epsilon^{abc} \, \epsilon_{def} = 3! \, h^{[a}{}_d \, h^b{}_e \, \delta^{c]}{}_f\\
&& \epsilon^{abc} \, \epsilon_{cef} = 2! \, h^{[a}{}_e \, h^{b]}{}_f\\
&& \epsilon^{abc} \, \epsilon_{bcf} = 2! \, h^a{}_f \\
&& \epsilon^{abc} \, \epsilon_{abc} = 3!
\end{eqnarray}
\end{subequations}
%

The projected covariant derivative, the time derivative, and the generalized 3-dimensional curl of tensors:
%
\begin{align}
\D_a T_{b\dots}{}^{c\dots} & \equiv h^d_a h^e_b \dots h^c_f \dots \nabla_d T_{e\dots}{}^{f\dots}\\
\dot T_{b\dots}{}^{c\dots} & \equiv  u^a \nabla_a T_{b\dots}{}^{c\dots}\\
\curl T_{ab\dots c} & \equiv \epsilon_{d e (a} \D^d {T_{b\dots c)}}^e
\end{align}
%
$\curl T_{ab\dots c}$ is PSTF for ${T_{ab\dots c}}$ PSTF \cite{Challinor:1999xz}. 
 

Kinematics are produced by taking the irreducible decomposition of the covariant derivative of the 4-velocity:
%
\begin{equation}
\nabla_a u_b = \frac{1}{3} \Theta h_{ab} + \sigma_{ab} + \omega_{ab} - u_a A_b
\label{velocity_decomp}
\end{equation} 
%
where:
%
\begin{align}
\Theta & \equiv \D^a u_a = 3H \label{expansion_def}\\
\sigma_{ab} =  \sigma_{(ab)} & \equiv\D_{\langle a} u_{b \rangle} \label{shear_def}\\
\omega_{ab} = \omega_{[ab]} & \equiv \D_{[a}u_{b]} \label{vorticity_def}\\
A_b & \equiv \dot u_b \label{acceleration_def}
\end{align}
%
are the expansion scalar, the shear, the vorticity, and the acceleration, respectively. $H$ is the local Hubble parameter. The parentheses/brackets denote symmetrization/anti-symmetrization over indices $a$ and $b$. The angle brackets denote the orthogonal projection of the symmetric trace free part of a tensor and defined as:
%
\begin{equation}
X_{\langle ab \rangle} \equiv \left[ h_{(a}{}^c \, h_{b)}{}^{d} - \frac{1}{3} \, h_{ab} \, h^{cd} \right] X_{cd}
\label{anglebracket_def}
\end{equation}
%
Another useful kinematic quatity is the projected vorticity vector, defined from the vorticity tensor by:
%
\begin{equation}
\omega_a \equiv \epsilon_{abc} \omega^{bc} /2 = \curl u_a /2
\label{vorticity_vec}
\end{equation}

Deriving directly from equations \eqref{expansion_def}--\eqref{acceleration_def}, we have:
%
\begin{align}
& u^a A_a = 0 \\
& u^a \sigma_{ab} = 0, \qquad \qquad \sigma^a{}_a = 0 \\
& u^a \omega_{ab} = 0, \qquad \qquad \omega^a{}_a = 0
\end{align}
%
which means that the shear and vorticity are PSTF. $A_a$ and $\sigma_{ab}$, and $\omega_a$ characterise anisotropy in the expansion. The projected gradient of the expansion scalar, $\D_a \Theta$, describes inhomogeneity in the expansion. These quantities all vanish in an exact FLRW universe \cite{Challinor:1999xz}.

The last term in the right hand side of Eq. \eqref{velocity_decomp} is the time component of the covariant derivative of the 4-velocity. The definitions in Eq. \eqref{expansion_def}~--~Eq. \eqref{vorticity_def} and Eq. \eqref{anglebracket_def} assert that the shear and expansion terms are the symmetric parts of the rest-space component of $\nabla_a u_b$ while the vorticity term is the antisymmetric part:
%
\begin{equation}
\D_a u_b =  \frac{1}{3} \Theta h_{(ab)} + \sigma_{(ab)} + \omega_{[ab]}
\end{equation}
%





%%%%%%%%%%%%%%%%%%%%%%%by hb
The tidal forces felt by a body moving along a geodesic are represented by the Riemann cuvature tensor, $R_{abcd}$, which may be decomposed into its trace and trace-free parts \cite{Ellis:2009go}:
%
\begin{equation}
R_{ab}{}^{cd} = 2 g_{[a}{}^{[c} \, R_{b]}{}^{d]} - \frac{R}{3} \, g_{[a}{}^{[c} \, g_{b]}{}^{d]} + C_{ab}{}^{cd}
\end{equation}
%
where $C_{abcd}$ is the Weyl tensor and describes the vacuum contribution to the gravitational field. It can be decomposed further into a curl-free and a divergence-free PSTF tensors:
 \begin{eqnarray}
E_{ab}  &\equiv&  u^c u^d C_{acbd} \\
H_{ab}  &\equiv&  \frac{1}{2} \, \epsilon_{acd} \, u^e C_{be}{}^{cd}
\end{eqnarray}
%
which are called the \emph{electric} and \emph{magnetic} Weyl tensors, in analogy with the curl-free electric field and divergence-free magnetic field in electromagnetism. $E_{ab}$ is analogous to the tidal tensor derived from the potential in Newtonian gravitation. $H_{ab}$ has no Newtonian counterpart thus is essential for a full description of gravitational waves \cite{Dunsby:1998hd}.

% ---------------------------------------------------------------------------
% ----------------------- end of thesis sub-document ------------------------
% ---------------------------------------------------------------------------

==> 9_backmatter/appendices/manifolds/manifolds.tex <==
The metric tensor is one very important, if not the most important, structure defined on a manifold:
%
\begin{equation}
g_{ab} \equiv \vec e_a \cdotp \vec e_b
\label{metric}
\end{equation}
%
where the vectors $\vec e_a$ are the basis of the manifold.

The covariant derivative on the manifold:
%
\begin{equation}
T_{abc\cdots;z} = T_{abc\cdots,z} - \Gamma^k_{\phantom kaz} T_{kbc\cdots}  - \Gamma^k_{\phantom kbz} T_{akc\cdots} - \cdots
\end{equation}
%
obviously requires the \emph{affine connection} \cite{Clifton:2011jh}:
%
\begin{equation}
\Gamma^a_{\phantom abc} \equiv  \{^a_{bc}\} + K^a_{\phantom abc} + L^a_{\phantom abc}
\label{Gamma} 
\end{equation}
%
where $\{^a_{bc}\}$ is the Levi-Civita connection defined in terms of the metric tensor:
%
\begin{equation}
\{^{a}_{bc}\} \equiv \frac{1}{2} g^{ad} (g_{bd,c} + g_{cd,b} - g_{bc,d})
\label{LCC} 
\end{equation}
%
$K^a_{\phantom a b c}$ is the contorsion tensor defined in terms of the anti-symmetric parts of the connection:
%
\begin{equation}
K^a_{\phantom a b c} \equiv \Gamma^a_{\phantom a [b c]} - \Gamma^d_{\phantom d [b e]} g^{ae} g_{cd} - \Gamma^d_{\phantom d [c e]} g^{ae} g_{bd}
\label{contorsion} 
\end{equation}
%
or in terms of the torsion tensor $T_{ab}^{\phantom{ab}c} \equiv 2 \Gamma^c_{\phantom c [ab]}$ \cite{ortin2007}:
\begin{equation}
K_{ab}^{\phantom{ab}c} \equiv \frac{1}{2} g^{cd} \l( T_{adb} + T_{bda} - T_{abd} \r) 
\label{contorsion2} 
\end{equation}
%
Finally, $L^a_{\phantom a b c}$ is defined in terms of the non-metricity tensor, $Q_{abc} \equiv \nabla_a g_{bc}$, as:
\begin{equation}
L^a_{\phantom a b c} \equiv \frac{1}{2} \l( Q^a_{\phantom a cb} - Q_{bc}^{\phantom{bc}a} - Q_{cb}^{\phantom{cb}a} \r) 
\label{contorsion2} 
\end{equation}

The GR spacetime is a four dimensional torsionless manifold that satisfies the \emph{metric postulate} $Q_{abc} = 0$. That is to say that both $K^a_{\phantom a b c}$ and $L^a_{\phantom a b c}$ vanish and the connection, which is now symmetric on the lower indices, reduces to the Levi-Civita connection which is completely defined by the metric tensor.

The curvature of a region on a manifold is described by the change of the order of the double covariant differentiation of a vector field:
%
\begin{equation}
v_{a;bc} - v_{a;cb} = R^d_{\phantom dabc} v_d
\label{vector_curv}
\end{equation}
%
where
%
\begin{equation}
R^d_{\phantom dabc} \equiv \Gamma^d_{\phantom dac,b} - \Gamma^d_{\phantom dab,c} + \Gamma^e_{\phantom eac} \Gamma^d_{\phantom deb} - \Gamma^e_{\phantom eab} \Gamma^d_{\phantom dec}
\end{equation}
%
is called the \emph{Riemann tensor} or the \emph{curvature tensor}, which obeys the following symmetries in the metric connection:
%
\begin{align}
& R_{abcd} = R_{cdab} &&\mathrm{Symmetry\ over\ the\ first\ and\ last\ pair\ of\ indices} \label{Riemann_sym}\\
& R_{abcd} = R_{[ab][cd]} &&\mathrm{Antisymmetry\ in\ the\ first\ and\ last\ pair\ of\ indices} \label{Riemann_anti_sym}\\
& R_{a[bcd]} = 0 &&\mathrm{Cyclic\ identities} \label{cyclic_id} \\
& R_{[ab|cd|;e]} = 0 &&\mathrm{Bianchi\ identities} \label{bianchi_id} 
\end{align}
%
The Bianchi identities are derived from the cyclic identities. Equation \eqref{vector_curv} is an important geometrical result for 4-vectors that will be used in deriving the Raychaudhuri equation \eqref{raychaudhuri}.

Contraction over the first and third indices of the Riemann tensor yields another curvature tensor dubbed the \emph{Ricci tensor}:
%
\begin{equation}
R_{ab} \equiv g^{cd} R_{cadb} = R^c_{\phantom cacb}
\end{equation}
%
Another contraction over the two indices of the Ricci tensor gives the \emph{Ricci scalar}:
%
\begin{equation}
R \equiv g^{ab} R_{ab} = R^a_a
\end{equation}
%
defined at every point of the manifold.

It is worth finishing by stating a relation of great importance in relativity. From the Bianchi identities (Eq. \ref{bianchi_id}), and using the symmetry relation (Eq. \ref{Riemann_anti_sym}) it follows that:
%
\begin{equation}
\l( R_{ab} - \frac{1}{2} g_{ab} R \r)^{;b} = 0
\end{equation}
%
The Einstein tensor $G_{ab} \equiv R_{ab} - \frac{1}{2} g_{ab} R$ is divergence free \cite{Hobson}.



==> 9_backmatter/appendices/sigma_2_u/custom_commands.tex <==
%%%%%%%%%%%%%%%%%%%% % Bourhrous % %%%%%%%%%%%%%%%%%%%%%%
\def \vec #1{\textbf{\em  #1}}
\newcommand{\Cl}{C_\ell}
\newcommand{\Pl}{P_\ell}
\newcommand{\cn}{/**citation needed**/}
%\newcommand{\l}{\ell}
%%%%%%%%%%%%%%%% % Leong % %%%%%%%%%%%%%%%%

\newcommand{\p}{\partial}
%\newcommand{\g}{\gamma}
\newcommand{\D}{\Delta}
\newcommand{\n}{\nabla}
\def\l{\left}
\def\r{\right}
\def\D{\Delta}
\def\dt{\cdot}
\def\w{\wedge}
\def\n{\nabla}
\newcommand{\hs}{\,-\,}
\newcommand \dd[2] {\frac{d {#1}}{d {#2}}}
\newcommand \pp[2] {\frac{\p {#1}}{\p {#2}}}
\newcommand \ppd[2] {\frac{\p^2 {#1}}{\p {#2}^2}}
\newcommand \ddp[2] {\frac{ d^2 {#1}}{d {#2}^2}}
\newcommand \bra[1] {\big< {#1}|}
\newcommand \ket[1] {| {#1} \big>}
\newcommand \ps {\mathcal{I}}
\newcommand{\nab}{\tilde{\nabla}}
\renewcommand{\theequation}{\arabic{equation}}
\def\mat#1  { \begin{matrix}#1\end{matrix} }
\def\pmat#1 { \begin{pmatrix}#1\end{pmatrix} }
\def\cas#1  { \begin{cases}#1\end{cases} }

%%%%%%%%%%%%%%%%% Commands from Ananda et. al %%%%%%%%%%%%
% 

\def \D {\tilde{\nabla}}
\def \ni {\noindent}
% \def\l{\label}
% \def\ct{\cite}
% \def\r{\ref}
% \def\lgth{[\,\mbox{length}\,]}
% \def\gam{\gamma}
% \def\del{\delta}
% \def\eps{\Epsilon}
% \def\Th{\Theta}
% \def\dd{\mathcal D}
% \def\zz{\mathcal Z}
% \def\sig{\sigma}
% \def\om{\omega}
% \def\udot{\dot{u}}
% \def\nab{\nabla}
\def\3nab{\tilde{\nabla}}
% \def\fd{{\bf e}}
% \def\p{\partial}
\def\lgl{\langle}
\def\rgl{\rangle}
% \def\la {\langle}
% \def\ra {\rangle}
\def\nn{\nonumber}
\def\c{\mbox{curl}}
% \def\div{\mbox{div}}
% \def\tl{\tilde}
% \def\hsp5{\hspace{5mm}}
% \newcommand{\sfrac}[2]{{\textstyle{#1\over#2}}}
% \def\case#1/#2{\textstyle\frac{#1}{#2}}
% \def\rd {\displaystyle{\cdot}}
% \def\ts {\textstyle}
% \def\be {\begin{equation}}
% \def\ee {\end{equation}}
% \def\ber {\begin{eqnarray}}
% \def\eer {\end{eqnarray}}
% \def\bea {\begin{eqnarray}}
% \def\eea {\end{eqnarray}}
% \def\cs{c_{s}^{2}}
% \def\ub {u_{\!_B}}
% \def\vb {v_{\!_B}}
% \def\eb {e_{\!_B}}
% \def\st {\sigma_{\!_T}}
% \def\ne {n_{\!_E}}
% \def\ts {\textstyle}
% \def\bc {\begin{center}}
% \def\ec {\end{center}}
% \newcommand{\hs}{\,-\,}
% \def\bi {\bibitem}
% %\def\case#1/#2{\textstyle\frac{#1}{#2} }
% \def\t {\textstyle}
% \def\jmp{{\it J. Math. Phys.}\ }
% \def\pr{{\it Phys. Rev.}\ }
% \def\jmp{{\it J. Math. Phys.}\ }
% \def\pr{{\it Phys. Rev.}\ }
% \def\prl{{\it Phys. Rev. Lett.}\ }
% \def\pl{{\it Phys. Lett.}\ }
% \def\np{{\it Nucl. Phys.}\ }
% \def\modpl{{\it Mod. Phys. Lett.}\ }
% \def\ijmp{{\it Int. Journ. Mod. Phys.}\ }
% \def\ijtp{{\it Int. Journ. Theor. Phys.}\ }
% \def\cmp{{\it Commun. Math. Phys.}\ }
% \def\cqg{{\it Class. Quantum Grav.}\ }
% \def\ap{{\it Ann. Phys. (N.Y.)}\ }
% \def\spj{{\it Sov. Phys. JETP}\ }
% \def\spjl{{\it Sov. Phys. JETP Lett.}\ }
% \def\prs{{\it Proc. R. Soc.}\ }
% \def\grg{{\it Gen. Relativ. Grav.}\ }
% \def\nat{{\it Nature}\ }
% \def\apj{{\it Ap. J.}\ }
% \def\aa{{\it Astron. Astrophys.}\ }
% \def\ncim{{\it Il Nuovo Cim.}\ }
% \def\ptp{{\it Prog. Theor. Phys.}\ }
% \def\aip{{\it Adv. Phys.}\ }
% \def\jpamg{{\it J. Phys. A: Math. Gen.}\ }
% \def\mnras{{\it Mon. Not. R. Ast. Soc.}\ }
% \def\prep{{\it Phys. Rep.}\ }
% \def\ncb{{\it Il Nuovo Cimento ``B''}}
% \def\ssr{{\it Space Sci. Rev.}\ }
% \def\pasp{{\it Pub. A. S. P.}\ }
% \def\araa{{\it Ann. Rev. Astr. Ap.}\ }
% \def\asr{{\it Adv. Space Res.}\ }
% \def\rmp{{\it Rev. Mod. Phys.}\ }
% \def\etal\;{{\it et al.}}
% \def\ie{{\it i.e. }}
% \def\eg{{\it e.g. }}
% \def\jmp{{\it J. Math. Phys.}\ }
% \def\lrr{{\it Liv. Rev. Rel.}\ }
% \def\nat{{\it Nature}\ }
% \def\apj{{\it Ap. J.}\ }
% \def\mnras{{\it Mon. Not. R. Ast. Soc.}\ }
% \def\araa{{\it Ann. Rev. Astr. Ap.}\ }
% \def\rmp{{\it Rev. Mod. Phys.}\ }
% \def\arns{{\it Ann. Rev. Nucl. Part. Sci.}\ }
% \newcommand{\n}{{}^{(3)}\nabla} \newcommand{\na}{\nabla}
% \newcommand{\hl}{\vspace{0.2cm}\hrule width\hsize height 0.45pt\vspace{0.2cm}}
% \newcommand{\da}{{\cal D}_a}
% \newcommand{\ft}{\left(\frac{t}{t_i}\right)}
% \newcommand{\0}{^{(0)}}
% \newcommand{\1}{^{(1)}}
% \newcommand{\2}{^{(2)}}
% \newcommand{\ab}{_{\alpha\beta}}
% \newcommand{\h}{\case{a'}/{a}}
% \newcommand{\inps}{\psi^{-1}}
% \newcommand{\ua}{\left(\frac{\nabla_a\phi}{\psi}\right)}
% \newcommand{\as}{{\cal A}}
% \newcommand{\bb}{{\cal B}}
% \newcommand{\cc}{{\cal C}}
% \newcommand{\es}{{\cal E}}
% \newcommand{\kk}{{\cal K}}
% \newcommand{\ls}{{\cal L}}
% \newcommand{\so}{{\cal O}}
% \newcommand{\sr}{{\cal R}}
% \newcommand{\ti}{\tilde}
% \newcommand{\wt}{\widetilde}
% \newcommand{\ii}{{(i)}}
% \newcommand{\jn}{{(j)}}
% \newcommand{\wcn}{\wt{C}_{(\nu)}}
% \newcommand{\dn}{\Delta_{(\nu)}}
% \newcommand{\pn}{\Phi_{(n)}}

% Challinor
\newcommand{\curl}{\,\mbox{curl}\,}
% \newcommand{\ord}{\mbox{O}}
% \newcommand{\sigt}{\sigma_{\mathrm{T}}}
% \newcommand{\nelec}{n_{\mathrm{e}}}
% \newcommand{\ud}{{\mathrm{d}}}
\newcommand{\Drm}{{\mathrm{D}}}
% \newcommand{\tc}{t_{\mathrm{c}}}
% \newcommand{\clq}{{\mathcal{Q}}}
% \newcommand{\TT}{{\mathrm{TT}}}
% \newcommand{\clh}{{\mathcal{H}}}
% \newcommand{\clp}{{\mathcal{P}}}

==> 9_backmatter/appendices/svt/svt_decomp.tex <==
\section{Scalar-Vector-Tensor Decomposition of the Perturbation Metric}
\label{svt_decomp}
The scalar-vector-tensor decomposition is based on the fact that any 3-vector can be expressed as the sum of its rotational and irrotational parts:
\begin{equation}
v_i = v_i^\parallel + v_i^\perp
\label{vec_decomp}
\end{equation}
such that $\D^i v_i^\perp = \curl v_i^\parallel = 0$. The irrotational, or longitudinal, vector can be written as the gradient of a scalar:
%
\begin{equation}
v_i^\parallel = \D_i\phi_v
\end{equation}
%
while the rotational, or transverse, part cannot be obtained from a scalar.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Similarly, a rank two tensor can be decomposed into a doubly longitudinal, a singly longitudinal, and a doubly transverse tensor:
%
\begin{equation}
S_{ij}=S_{ij}^\parallel+S_{ij}^\perp+S_{ij}^{\rm T}\ ,
\label{tensor_decomp}
\end{equation}
%
such that 
%
\begin{equation}
\D^j S_{ij} = \D^j S_{ij}^\parallel + \D^j S_{ij}^\perp\ .
\label{tensor_div}
\end{equation}
%
The divergence of the doubly transverse component is zero. For $S_{ij}$ PSTF, the doubly and singly longitudinal parts can be
obtained from the gradients of a scalar and a transverse vector:
\begin{equation}
  S_{ij}^\parallel = \l( \D_i \D_j - \frac{1}{3} h_{ij} \D^2 \r) \phi_S \ ,\quad S_{ij}^\perp = 2 \D_{(i} S_{j)}^\perp .
  \label{longtens}
\end{equation}

The perturbed metric, in linear perturbation theory, can be regarded as a symmetric tensor $\xi_{ab}$ on adding to the FLRW metric:
%
\begin{equation}
g_{ab} = g_{ab}^{\mathrm{FLRW}} + \xi_{ab}
\end{equation}
%
with:
%
\begin{equation}
  \xi_{00} \equiv - 2 \psi\ , \quad
  \xi_{0i}\equiv v_i\ , \quad
  \xi_{ij} \equiv 2 \l( \phi h_{ij} + S_{ij} \r)
  \label{pertur_tensor}
\end{equation}
%
and $S^i_{\phantom ii}=0$.

scalar represent density perturbations.

vector is gravitomagnetism

tensor modes are gravitational waves.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\cite{Bertschinger:2001is}

% In linear perturbation theory, the metric perturbations $h_{\mu\nu}$
% are regarded as a tensor field residing on the background
% Robertson-Walker spacetime.  As a symmetric $4\times4$ matrix,
% $h_{\mu\nu}$ has 10 degrees of freedom.  Because of the ability
% to make continuous deformations of the coordinates, 4 of these
% degrees of freedom are gauge- (coordinate-) dependent, leaving
% 6 physical degrees of freedom.  A proper treatment of cosmological
% perturbation theory requires clear separation between physical and
% gauge degrees of freedom.
% 
% The metric degrees of freedom in linear pertubation theory were
% classified by Lifshitz in 1946 [\cite{lifsh}].  Lifshitz presented
% the scalar-vector-tensor decomposition of the metric.  It is based
% on a $3+1$ split of the components, which we rewrite as follows:
% \begin{equation}
%   h_{00}\equiv-2\psi\ ,\quad
%   h_{0i}\equiv v_i\ ,\quad
%   h_{ij}=2\left(\phi\gamma_{ij}+S_{ij}\right)\
%     \hbox{with \gamma^{ij}S_{ij}=0.}
%   \label{3p1}
% \end{equation}
% Here, $\gamma^{ij}$ is the matrix inverse of $\gamma_{ij}$.
% The trace part of $h_{ij}$ has been absorbed into $\phi$ so
% that $S_{ij}$ has only 5 independent components.
%  
% With the space-time ($3+1$) split, we use $\gamma_{ij}$
% (or $\gamma^{ij}$) to lower (or raise) indices of spatial 3-vectors
% and tensors.  For convenience, spatial derivatives will be
% written using the 3-dimensional covariant derivative $\D_i$
% defined with respect to the 3-metric $\gamma_{ij}$; it is a
% three-dimensional version of the full 4-dimensional covariant
% derivative presented in general relativity textbooks.  For example,
% if $K=0$, we can choose Cartesian coordinates such that $\gamma_{ij}=
% \delta_{ij}$ and $\D_i=\partial/\partial x^i$.
% 
% The scalar-tensor-vector split is based on the decomposition of a vector
% into longitudinal and transverse parts.  For any three-vector field
% $v_i(\vec x\,)$, we may write
% \begin{equation}
%   v_i=v_i^\parallel+v_i^\perp\quad\hbox{where}\ \vec\D\times
%     \vec w^{\,\parallel}=\vec\D\cdot\vec w^{\,\perp}=0\ .
%   \label{ltsvec}
% \end{equation}
% The curl and divergence are defined using the spatial covariant
% derivative, e.g. $\vec\D\cdot\vec w=\gamma^{ij}\D_iw_j$.
% 
% The longitudinal/transverse decomposition is not unique (e.g. one may
% always add a constant to $v_i^\parallel$) but it always exists.  The
% terminology arises because in the Fourier domain $v_i^\parallel$ is
% parallel to the wavevector while $v_i^\perp$ is transverse (perpendicular
% to the wavevector).  Note that $v_i^\parallel=\D_i\phi_w$ for some
% scalar field $\phi_w$.  Thus, the longitudinal/transverse decomposition
% allows us to write a vector field in terms of a scalar (the longitudinal
% or irrotational part) and a part that cannot be obtained from a scalar
% (the transverse or rotational part).
% 
% A similar decomposition holds for a two-index tensor, but now each index
% can be either longitudinal or transverse.  For a symmetric tensor, there
% are three possibilities: both indices are longitudinal, one is transverse,
% or two are transverse.  These are written as follows:
% \begin{equation}
%   S_{ij}=S_{ij}^\parallel+S_{ij}^\perp+S_{ij}^{\rm T}\ ,
%   \label{ltsten}
% \end{equation}
% where
% \begin{equation}
%   \gamma^{jk}\D_kS_{ij}=\gamma^{jk}\D_kS_{ij}^\parallel+
%     \gamma^{jk}\D_kS_{ij}^\perp\ .
%   \label{divtens}
% \end{equation}
% The first term in equation (\ref{divtens}) is a longitudinal vector
% while the second term is a transverse vector.  The divergence of the
% doubly-transverse part, $S_{ij}^{\rm T}$, is zero.  For a traceless
% symmetric tensor, the doubly and singly longitudinal parts can be
% obtained from the gradients of a scalar and a transverse vector,
% respectively:
% \begin{equation}
%   S_{ij}^\parallel=\left(\D_i\D_j-{1\over3}\gamma_{ij}
%     \D^2\right)\phi_S\ ,\quad
%   S_{ij}^\perp=\D_iS_j^\perp+\D_jS_i^\perp\ .
%   \label{longtens}
% \end{equation}
% 
% Although we will not prove it here (see [\cite{lesh}] for the details),
% under an infinitesimal coordinate transformation $S_{ij}^\parallel$
% and $S_{ij}^\perp$ can change while $S_{ij}^{\rm T}$ is invariant.
% Similarly, the longitudinal and transverse parts of $v_i=h_{0i}$
% are both gauge-dependent.
% 
% Now we have the mathematical background needed to perform the
% scalar-tensor-vector split of the physical degrees of freedom
% of the metric.  The ``tensor mode'' represents the part of $h_{ij}$
% that cannot be obtained from the gradients of a scalar or
% vector, namely $S_{ij}^{\rm T}$.  The tensor mode is gauge-invariant
% and has two degrees of freedom (five for a symmetric traceless
% $3\times3$ matrix, less three from the condition $\gamma^{jk}
% \D_kS_{ij}^{\rm T}=0$).  Physically it represents gravitational
% radiation; the two degrees of freedom correspond to the two
% polarizations of gravitational radiation.  Gravitational radiation
% is transverse: a wave propagating in the $z$-direction can have
% nonzero components $h_{xx}-h_{yy}$ and $h_{xy}=h_{yx}$ but no others.
% The tensor mode $S_{ij}^{\rm T}$ behaves like a spin-2 field under
% spatial rotations.  Note that my definition of the tensor mode
% strain $S_{ij}$ here differs by a factor of 2 from the conventional
% $h_{ij}^{TT}$ in [\cite{mtw}].
% 
% The ``vector mode'' behaves like a spin-1 field under spatial
% rotations.  It corresponds to the transverse vector parts of the
% metric, which are found in $v_i^\perp$ and $S_{ij}^\perp$.  Each
% part has two degrees of freedom.  Although we will not prove it
% here (see [\cite{lesh}] for the details), it is possible to eliminate
% two of these degrees of freedom by imposing gauge conditions
% (coordinate conditions).  The synchronous gauge of Lifshitz
% [\cite{lifsh}] is one popular choice, with $v_i^\perp=v_i^\parallel=0$.
% Another choice is the ``Poisson'' or transverse gauge [\cite{lesh}]
% which sets $S_{ij}^\perp=0$.  In either case, there are two
% physical degrees of freedom and they correspond physically
% to gravitomagnetism.  Although this effect is less well known than
% gravitational radiation or Newtonian gravity, it produces magnetic-like
% effects on moving and spinning masses, such as the precession of a
% gyroscope in the gravitational field of a spinning mass (Lense-Thirring
% precession).  This phenomenon has not yet been discovered experimentally
% but should be measured by the Gravity Probe B satellite to be launched
% in 2002 [\cite{gpb}].
% 
% The ``scalar mode'' is spin-0 under spatial rotations and corresponds
% physically to Newtonian gravitation with relativistic modifications.
% The scalar parts of the metric are given by $\phi$, $\psi$,
% $v_i^\parallel$, and $S_{ij}^\parallel$.  Any two of these may
% be set to zero by means of a gauge transformation.  One popular choice
% is $v_i^\parallel=S_{ij}^\parallel=0$, also known as the conformal
% Newtonian gauge.  It corresponds to the scalar mode in the {\bf transverse
% gauge}, defined by the gauge conditions
% \begin{equation}
%   \gamma^{ij}\D_iw_j=0\ ,\quad
%   \gamma^{jk}\D_kS_{ij}=0\ .
%   \label{transg}
% \end{equation}
% This gauge in linearized general relativity is the gravitational
% analogue of Coulomb gauge in electromagnetism, where the magnetic
% vector potential is transverse, $\D_iA^i=0$.  In the gravitational
% transverse gauge, $v_i$ is transverse and $S_{ij}$ is doubly transverse.
% This gauge is convenient for developing intuition although not necessarily
% the best for computation.  The variables $(\phi,\psi,v_i^\perp,
% S_{ij}^{\rm T})$ correspond to gauge-invariant variables introduced
% by Bardeen [\cite{bard}] as linear combinations of metric variables
% in other gauges.
% 
% In linear perturbation theory, the scalar, vector, and tensor modes
% evolve independently.  The vector and tensor modes produce no density
% perturbations and therefore are unimportant for structure formation,
% although they do perturb the microwave background.  In the remainder
% of these lectures, only the scalar mode will be considered.
% 
% The Einstein equations give the equations of motion for the metric
% perturbations in terms of the energy-momentum tensor, the source of
% relativistic gravity.  Here we consider the case of a perfect fluid
% (or several perfect fluid components combined), for which
% \begin{equation}
%   T^{\mu\nu}=(\rho+p)V^\mu V^\nu+pg^{\mu\nu}
%   \label{tmunu}
% \end{equation}
% where $\rho$ and $p$ are the proper energy density and pressure in
% the fluid rest frame and $V^\mu$ is the fluid 4-velocity.
% 
% We split $T^{\mu\nu}$ into time and space components as we did for the
% metric.  It is convenient to use mixed components because the conformal
% factor $a^2$ then cancels, yielding
% \begin{eqnarray}
%   \label{tcompon}
%   T^0_{\ \,0}&=&-\rho(\vec x,\tau)=-\left[\bar\rho(\tau)+\delta
%     \rho(\vec x,\tau)\right]\ ,\nonumber \\
%   T^0_{\ \,i}&=&\left[\bar\rho(\tau)+\bar p(\tau)\right]v_i(\vec x,\tau)
%     =-\left[\bar\rho(\tau)+\bar p(\tau)\right]\D_i W\ ,\\
%   T^i_{\ \,j}&=&\left[\bar p(\tau)+\delta p(\vec x,\tau)\right]
%     \delta^i_{\ \,j}\ ,\nonumber
% \end{eqnarray}
% where $\bar\rho(\tau)$ and $\bar p(\tau)$ are respectively the energy
% (or mass) density and pressure of the Robertson-Walker background
% spacetime, $v_i=\gamma_{ij}dx^j/d\tau$ is the fluid 3-velocity
% (assumed nonrelativistic), and $W$ is a velocity potential.  We are
% assuming that the velocity field is irrotational or, if it is not,
% that the matter fluctuations are linear so that the longitudinal
% and transverse velocity components evolve independently.  This is
% a good approximation prior to the epoch of galaxy formation.
% 
% We are also making another approximation, namely that the shear
% stress (the non-diagonal part of $T^i_{\ \,j}$) is negligible
% compared with the pressure.  This is a bad approximation for
% relativistic neutrinos, whose free-streaming leads to a non-isotropic
% momentum distribution after neutrino decoupling at a temperature
% of about 1 MeV.  (A similar but smaller effect occurs for photons
% after they decouple at a temperature of about 0.3 eV.)  However,
% the effect of this error is modest during the radiation-dominated
% era (photons contribute more pressure than neutrinos, and are
% isotropic) and is unimportant during the matter-dominated era,
% when the nonrelativistic matter density is the major source of
% gravity.  We introduce this approximation here in order to
% simplify the treatment; full calculations include the effects of
% neutrino shear stress [\cite{mabert}].
% 
% When the stress tensor is isotropic, the Einstein equations in
% transverse gauge imply that the two scalar potentials $\phi$ and
% $\psi$ are equal [\cite{lesh}] and the metric takes the simple form
% \begin{equation}
%   ds^2=a^2(\tau)\left[-(1+2\phi)d\tau^2+(1-2\phi)\gamma_{ij}dx^idx^j
%     \right]\ .
%   \label{cnmet}
% \end{equation}
% This is a simple cosmological generalization of the standard weak-field
% limit of general relativity, which is recovered by setting $a=1$ and
% $\gamma_{ij}=\delta_{ij}$.
% 
% Given the stress-energy tensor, we can now obtain field equations for
% $\phi(\vec x,\tau)$ using the Einstein equations.  The only independent
% equation for the Robertson-Walker background is the Friedmann equation
% (\ref{friedmann}).  For the perturbations, we obtain
% \begin{equation}
%   \label{poisson}
%   (\D^2+3K)\phi=4\pi Ga^2\left[\delta\rho+3{\dot a\over a}(\bar\rho
%     +\bar p)W\right]\ ,
% \end{equation}
% \begin{equation}
%   \label{momcon}
%   \partial_\tau\phi+{\dot a\over a}\phi=4\pi Ga^2(\bar\rho+\bar p)W\ ,
% \end{equation}
% and
% \begin{equation}
%   \label{phidd}
%   \partial_\tau^2\phi+3{\dot a\over a}\partial_\tau\phi-\left(
%     8\pi Ga^2\bar p+2K\right)\phi=4\pi Ga^2\delta p\ .
% \end{equation}
% There are more equations than in Newtonian gravity because the
% Einstein equations have local energy-momentum conservation built
% into them.
% 
% Equation (\ref{poisson}) is remarkably like the Poisson equation of
% Newtonian gravity, especially when one realizes that the factor of
% $a^2$ is needed to convert the Laplacian from comoving to proper
% spatial coordinates.  Otherwise there are three differences.  First,
% the spatial curvature adds a scale to the Laplacian in a curved space.
% Second,  the density source is $\delta\rho=\rho-\bar\rho$ rather
% than $\rho$ because $\phi$ represents a metric perturbation on top
% of the background Robertson-Walker spacetime.  Third, momentum density
% (through $W$) is a source for gravity in general relativity.
% However, this term is comparable with the density term only on
% length scales comparable to or larger than the Hubble length $H^{-1}$.
% 
% Two of our field equations are unfamiliar from Newtonian dynamics.
% Equation (\ref{momcon}) is reminiscent of the Zel'dovich approximation
% [\cite{za}] in that the velocity potential is proportional to the
% gravitational potential in the linear regime when $\phi(\vec x,\tau)=
% \phi_0(\vec x\,)D_\phi(\tau)$.  However, it is a more general result
% whose Newtonian limit may be derived by combining the continuity
% equation with the time derivative of the Poisson equation.
% 
% Equation (\ref{phidd}) is more surprising, as it gives the
% gravitational potential through a second-order time evolution
% equation as opposed to the action-at-a-distance Poisson equation
% (\ref{poisson}).  The reader may well wonder about the compatibility
% of the two equations as well as the physical validity of the Poisson
% equation in general relativity, but equations (\ref{poisson})--(\ref
% {phidd}) are all correct.  See [\cite{lesh}] for a full discussion.
% In brief, causality is restored by the tensor mode.  The time
% evolution equation for the potential can be regarded as arising
% from local energy-momentum conservation (which is built into the
% Einstein equations) combined with the Poisson equation.  Indeed,
% an equation similar to equation (\ref{phidd}) can be derived in
% Newtonian gravity from the fluid and Poisson equations.  Its utility
% arises from the fact that when pressure perturbations are
% gravitationally unimportant (i.e. when matter and/or dark energy
% dominate over radiation), the time evolution of perturbations can
% be obtained from a single differential equation depending only on
% the background curvature, pressure, and density.


==> 9_backmatter/appendices/svt/svt_harmonics.tex <==
Spatial harmonics are eigenfunctions of the Laplace-Beltrami operator, i.e.:
\begin{equation}
\D^2 Q = - \frac{k^2}{a^2} Q
\label{LBeq}
\end{equation}
%
and are, by construction, covariantly constant:
%
\begin{equation}
\dot Q = 0
\end{equation}
%
where $k = \frac{2 \pi a}{\lambda}$ is the wave number and $Q$ represents scalar $\l( Q^{(0)} \r)$, vector $\l( Q^{(1)}_a \r)$, or tensor $\l( Q^{(2)}_{ab} \r)$ harmonics \cite{Bruni:1992dg,Harrison:1967zz}.

Because different modes are independent, first order quantities $X(t,x)$ can be decomposed to or reconstructed from its harmonics via:
%
\begin{equation}
    X(t,x) = \sum X^{(k)}(t) Q^{(k)}(x)
\end{equation}
%
assuming that the quantity $X$ is factorizable intro purely temporal and spatial components \cite{Carloni:2007yv}.

==> 9_backmatter/appendices/svt_harmonics/svt_harmonics.tex <==
Spatial harmonics are eigenfunctions of the Laplace-Beltrami operator, i.e.:
\begin{equation}
\D^2 Q = - \frac{k^2}{a^2} Q
\label{LBeq}
\end{equation}
%
and are, by construction, covariantly constant:
%
\begin{equation}
\dot Q = 0
\end{equation}
%
where $k = \frac{2 \pi a}{\lambda}$ is the wave number and $Q$ represents scalar $\l( Q^{(0)} \r)$, vector $\l( Q^{(1)}_a \r)$, or tensor $\l( Q^{(2)}_{ab} \r)$ harmonics \cite{Bruni:1992dg,Harrison:1967zz}.

Because different modes are independent, first order quantities $X(t,x)$ can be decomposed to or reconstructed from its harmonics via:
%
\begin{equation}
    X(t,x) = \sum X^{(k)}(t) Q^{(k)}(x)
\end{equation}
%
assuming that the quantity $X$ is factorizable intro purely temporal and spatial components \cite{Carloni:2007yv}.

==> Latex/Classes/urlbst <==
#! /usr/bin/env perl
#
# Usage: ./urlbst.pl [--eprint] [--doi]
#    [--nohyperlinks] [--inlinelinks] [--hypertex] [--hyperref]
#    [input-file [output-file]]
# If either input-file or output-file is omitted, they are replaced by
# stdin or stdout respectively.
#
# See http://purl.org/nxg/dist/urlbst for documentation
#
# $Id: urlbst.in,v 1.8 2007/03/26 17:21:56 norman Exp $

$version = '0.6';
($progname = $0) =~ s/.*\///;
$mymarker = "% $progname";
$mymarkerend = "% ...$progname to here";
$myurl = 'http://purl.org/nxg/dist/urlbst';


$infile = '-';
$outfile = '-';

$addeprints = 0;     # if true (nonzero) we add support for eprints
$eprintprefix = 'arXiv:';	# make these settable with --eprint? syntax?
$eprinturl = 'http://arxiv.org/abs/';

$adddoiresolver = '0';
$doiprefix = 'doi:';
$doiurl = 'http://dx.doi.org/';

$makehref = 0;
$availablestring = "Available from: ";
$inlinelinks = 0;

$Usage = "$progname [--eprint] [--doi]\n    [--nohyperlinks] [--inlinelinks] [--hypertex] [--hyperref]\n    [--help] [input-file [output-file]]";

while ($#ARGV >= 0) {
    if ($ARGV[0] eq '--eprint') {
	$addeprints = 1;
    } elsif ($ARGV[0] eq '--doi') {
        $adddoiresolver = 1;
    } elsif ($ARGV[0] eq '--nohyperlinks') {
        $makehref = 0;
    } elsif ($ARGV[0] eq '--hypertex') {
	$makehref = 1;
    } elsif ($ARGV[0] eq '--hyperref') {
	$makehref = 2;
    } elsif ($ARGV[0] eq '--inlinelinks') {
        $inlinelinks = 1;
    } elsif ($ARGV[0] eq '--help') {
        print <<EOD;
urlbst version $version
    Usage: $Usage
      --eprint:       include support for `eprint' fields
      --doi:          include support for `doi' field
      --nohyperlinks  do not include active links anywhere
      --inlinelinks   add hyperlinks to entry titles
      --hypertex:     include HyperTeX-style hyperlink support
      --hyperref:     include {hyperref}-style hyperlink support
                      (generally better)
      --help:         print this help
    Input and output files may be given as `-' (default) to indicate stdin/out
EOD
        exit(0);
    } elsif ($ARGV[0] =~ /^-/) {
        die "Unrecognised option $ARGV[0]: Usage: $Usage\n";
    } elsif ($infile eq '-') {
	$infile = $ARGV[0];
    } elsif ($outfile eq '-') {
	$outfile = $ARGV[0];
    } else {
	die "Usage: $Usage\n";
    }
    shift(@ARGV);
}

if ($inlinelinks && $makehref == 0) {
    print <<'EOD';
Warning: --inlinelinks and --nohyperlinks were both specified (possibly
    implicitly).  That combination makes no sense, so I'll ignore
    --nohyperlinks and use --hyperref instead
EOD
    $makehref = 2;
}

$exitstatus = 0;		# success status

open (IN, "<$infile") || die "Can't open $infile to read";
open (OUT, ">$outfile") || die "Can't open $outfile to write";

# We have to make certain assumptions about the source files, in order
# to patch them at the correct places.  Specifically, we assume that
#
#   - there's a function init.state.consts
#
#   - ...and an output.nonnull which does the actual outputting, which
#         has the `usual' interface.
#
#   - we can replace
#           fin.entry
#       by
#           new.block
#           output.url    % the function which formats and displays any URL
#           fin.entry
#
#   - there is a function which handles the `article' entry type (this
#         will always be true)
#
#   - there is a function output.bibitem which is called at the
#         beginning of each entry type
#   - ...and one called fin.entry which is called at the end
#
# If the functions format.date, format.title or new.block are not defined (the
# former is not in apalike, for example, and the last is not in the
# AMS styles), then replacements are included in the output.
#
# All these assumptions are true of the standard files and, since most
# style files derive from them more or less directly, are true of most (?)
# other style files, too.
#
# There's some rather ugly Perl down here.  The parsing for
# brace-matching could probably do with being rewritten in places, to
# make it less ugly, and more robust.

print OUT "%%% Modification of BibTeX style file ", ($infile eq '-' ? '<stdin>' : $infile), "\n";
print OUT "%%% ... by $progname, version $version (marked with \"$mymarker\")\n%%% See <$myurl>\n";
print OUT "%%% Added webpage entry type, and url and lastchecked fields.\n";
print OUT "%%% Added eprint support.\n"   if ($addeprints);
print OUT "%%% Added DOI support.\n"      if ($adddoiresolver);
print OUT "%%% Added HyperTeX support.\n" if ($makehref == 1);
print OUT "%%% Added hyperref support.\n" if ($makehref == 2);
print OUT "%%% Original headers follow...\n\n";

$found{initconsts} = 0;
$found{outputnonnull} = 0;
$found{article} = 0;
$found{outputbibitem} = 0;
$found{finentry} = 0;
$found{formatdate} = 0;
$found{formattitle} = 0;
$found{newblock} = 0;

while (<IN>) {
    /^ *%/ && do {
        # Pass commented lines unchanged
        print OUT;
        next;
    };
    
    /^ *ENTRY/ && do {
	# Work through the list of entry types, finding what ones are there.
	# If we find a URL entry there already, object, since these edits
	# will mess things up.
	$line = $_;
	until ($line =~ /\{\s*(\w*)/) {
	    $line .= <IN>;
	}
	$bracematchtotal = 0;	# reset
	bracematcher($line);
	$line =~ /\{\s*(\w*)/;
	$found{'entry'.$1} = 1;
	print OUT $line;
	$line = <IN>;
	until (bracematcher($line) == 0) {
	    # XXX deal with multiple entries on one line
	    ($line =~ /^\s*(\w*)/) && ($found{'entry'.$1} = 1);
	    print OUT $line;
	    $line = <IN>;
	}
	if (defined($found{entryurl})) {
	    print STDERR "$progname: style file $infile already has URL entry!\n";
	    # print out the rest of the file, and give up
            print OUT $line;
	    while (<IN>) {
		print OUT;
	    }
	    $exitstatus = 1;
	    last;
	} else {
            print OUT "    eprint $mymarker\n    doi $mymarker\n    url $mymarker\n    lastchecked $mymarker\n";
	}
	print OUT $line;
	next;
    };

    /^ *FUNCTION *\{init\.state\.consts\}/ && do {
        # In the init.state.consts function, add an extra set of
        # constants at the beginning.  Also use this as the marker for
        # the place to add the init strings function.
        print OUT <<EOD;
STRINGS { urlintro eprinturl eprintprefix doiprefix doiurl openinlinelink closeinlinelink } $mymarker...
INTEGERS { hrefform inlinelinks makeinlinelink addeprints adddoiresolver }
% Following constants may be adjusted by hand, if desired
FUNCTION {init.urlbst.variables}
{
  "$availablestring" 'urlintro := % prefix before URL
  "$eprinturl" 'eprinturl := % prefix to make URL from eprint ref
  "$eprintprefix" 'eprintprefix := % text prefix printed before eprint ref
  "$doiurl" 'doiurl := % prefix to make URL from DOI
  "$doiprefix" 'doiprefix :=      % text prefix printed before DOI ref
  #$addeprints 'addeprints :=         % 0=no eprints; 1=include eprints
  #$adddoiresolver 'adddoiresolver :=     % 0=no DOI resolver; 1=include it
  #$makehref 'hrefform :=           % 0=no crossrefs; 1=hypertex xrefs; 2=hyperref refs
  #$inlinelinks 'inlinelinks :=        % 0=URLs explicit; 1=URLs attached to titles
  % the following are internal state variables, not config constants
  #0 'makeinlinelink :=     % state variable managed by setup.inlinelink
  "" 'openinlinelink :=     % ditto
  "" 'closeinlinelink :=    % ditto
}
INTEGERS { 
  bracket.state
  outside.brackets
  open.brackets
  within.brackets
  close.brackets
}
$mymarkerend
EOD
	$line = $_;
	until ($line =~ /\{.*\}.*\{/s) {
	    $line .= <IN>;
	}
	$line =~ s/(\{.*?\}.*?\{)/$1 #0 'outside.brackets := $mymarker
  #1 'open.brackets :=
  #2 'within.brackets :=
  #3 'close.brackets :=

 /s;
	print OUT $line;
	$found{initconsts} = 1;
	next;
    };

    /^ *EXECUTE *\{init\.state\.consts\}/ && do {
        print OUT "EXECUTE {init.urlbst.variables}\n";
        print OUT;
        next;
    };

    /^ *FUNCTION *\{new.block\}/ && do {
        $found{newblock} = 1;
    };

    /^ *FUNCTION *{output\.nonnull}/ && do {
	print OUT "$mymarker\n";
	print OUT "FUNCTION {output.nonnull.original}\n";
        copy_block();
	print_output_functions();
	$found{outputnonnull} = 1;
	next;
    };

    /FUNCTION *\{fin.entry\}/ && do {
        # Rename fin.entry to fin.entry.original (wrapped below)
        s/fin.entry/fin.entry.original/;
        $found{finentry} = 1;
        print OUT;
        next;
    };

    /^ *FUNCTION *{format\.date}/ && do {
	$found{formatdate} = 1;
	print OUT;
	next;
    };

    /^ *FUNCTION *{format\.title}/ && do {
        # record that we found this
	$found{formattitle} = 1;
        print OUT;
	next;
    };

    /^ *format\.b?title/ && do {
        # interpolate a call to setup.inlinelink
        print OUT "  title empty\$ 'skip\$ 'setup\.inlinelink if\$ $mymarker\n";
        print OUT;
        next;
    };

    /^ *FUNCTION *\{article\}/ && do {

	print_missing_functions();
	print_webpage_def();

	print OUT;
	$found{article} = 1;
	next;
    };

    /FUNCTION *\{output.bibitem\}/ && do {
        # Rename output.bibitem to output.bibitem.original (wrapped below)
        s/{output.bibitem\}/\{output.bibitem.original\}/;
 	$found{outputbibitem} = 1;
        print OUT;
        next;
    };

    print OUT;
};

if ($exitstatus == 0) {
    # Skip this if we've already reported an error -- it'll only be confusing
    foreach $k (keys %found) {
        if ($found{$k} == 0) {
            print STDERR "$progname: $infile: failed to find feature $k\n";
        }
    }
}

close (IN);
close (OUT);

exit $exitstatus;;






sub print_output_functions {
    print OUT "$mymarker...\n";

    print OUT <<'EOD';
% The following three functions are for handling inlinelink.  They wrap
% a block of text which is potentially output with write$ by multiple
% other functions, so we don't know the content a priori.
% They communicate between each other using the variables makeinlinelink
% (which is true if a link should be made), and closeinlinelink (which holds
% the string which should close any current link.  They can be called
% at any time, but start.inlinelink will be a no-op unless something has
% previously set makeinlinelink true, and the two ...end.inlinelink functions
% will only do their stuff if start.inlinelink has previously set
% closeinlinelink to be non-empty.
FUNCTION {setup.inlinelink}
{ makeinlinelink
    { hrefform #1 = % hypertex
        { "\special {html:<a href=" quote$ * url * quote$ * "> }{" * 'openinlinelink :=
          "\special {html:</a>}" 'closeinlinelink :=
          }
        { hrefform #2 = % hyperref
            { "\href{" url * "}{" * 'openinlinelink :=
              "}" 'closeinlinelink :=
              }
            'skip$
          if$ % hrefform #2 =
        }
      if$ % hrefform #1 =
      #0 'makeinlinelink :=
    }
    'skip$
 if$ % makeinlinelink
}
FUNCTION {add.inlinelink}
{ openinlinelink empty$
    'skip$
    { openinlinelink swap$ * closeinlinelink *
      "" 'openinlinelink :=
      }
  if$
}
EOD

    # new.block is defined elsewhere

    print OUT <<'EOD';
FUNCTION {output.nonnull}
{ % Save the thing we've been asked to output
  's :=
  % If the bracket-state is close.brackets, then add a close-bracket to
  % what is currently at the top of the stack, and set bracket.state
  % to outside.brackets
  bracket.state close.brackets =
    { "]" *
      outside.brackets 'bracket.state :=
    }
    'skip$
  if$
  bracket.state outside.brackets =
    { % We're outside all brackets -- this is the normal situation.
      % Write out what's currently at the top of the stack, using the
      % original output.nonnull function.
      s
      add.inlinelink
      output.nonnull.original % invoke the original output.nonnull
    }
    { % Still in brackets.  Add open-bracket or (continuation) comma, add the
      % new text (in s) to the top of the stack, and move to the close-brackets
      % state, ready for next time (unless inbrackets resets it).  If we come
      % into this branch, then output.state is carefully undisturbed.
      bracket.state open.brackets =
        { " [" * }
        { ", " * } % bracket.state will be within.brackets
      if$ 
      s * 
      close.brackets 'bracket.state :=
    }
  if$
}

% Call this function just before adding something which should be presented in 
% brackets.  bracket.state is handled specially within output.nonnull.
FUNCTION {inbrackets}
{ bracket.state close.brackets =
    { within.brackets 'bracket.state := } % reset the state: not open nor closed
    { open.brackets 'bracket.state := }
  if$
}

FUNCTION {format.lastchecked}
{ lastchecked empty$
    { "" }
    { inbrackets "cited " lastchecked * }
  if$
}
EOD
    print OUT "$mymarkerend\n";
}

sub print_webpage_def {
    print OUT "$mymarker...\n";

    # Some of the functions below call new.block, so we need a dummy
    # version, in the case where the style being edited doesn't supply
    # that function.
    if (! $found{newblock}) {
        print OUT "FUNCTION {new.block} % dummy new.block function\n{\n  % empty\n}\n\n";
        $found{newblock} = 1;
    }

    print OUT <<'EOD';
% Functions for making hypertext links.
% In all cases, the stack has (link-text href-url)
%
% make 'null' specials
FUNCTION {make.href.null}
{
  pop$
}
% make hypertex specials
FUNCTION {make.href.hypertex}
{ 
  "\special {html:<a href=" quote$ *
  swap$ * quote$ * "> }" * swap$ *
  "\special {html:</a>}" *
}
% make hyperref specials
FUNCTION {make.href.hyperref}
{ 
  "\href {" swap$ * "} {\path{" * swap$ * "}}" *
}
FUNCTION {make.href}
{ hrefform #2 =
    'make.href.hyperref      % hrefform = 2
    { hrefform #1 =
        'make.href.hypertex  % hrefform = 1
        'make.href.null      % hrefform = 0 (or anything else)
      if$
    }
  if$
}

% If inlinelinks is true, then format.url should be a no-op, since it's
% (a) redundant, and (b) could end up as a link-within-a-link.
FUNCTION {format.url}
{ inlinelinks #1 = url empty$ or
   { "" }
   { hrefform #1 =
       { % special case -- add HyperTeX specials
         urlintro "\url{" url * "}" * url make.href.hypertex * }
       { urlintro "\url{" * url * "}" * }
     if$
   }
  if$
}

FUNCTION {format.eprint}
{ eprint empty$
    { "" }
    { eprintprefix eprint * eprinturl eprint * make.href }
  if$
}

FUNCTION {format.doi}
{ doi empty$
    { "" }
    { doiprefix doi * doiurl doi * make.href }
  if$
}

% Output a URL.  We can't use the more normal idiom (something like
% `format.url output'), because the `inbrackets' within
% format.lastchecked applies to everything between calls to `output',
% so that `format.url format.lastchecked * output' ends up with both
% the URL and the lastchecked in brackets.
FUNCTION {output.url}
{ url empty$
    'skip$ 
    { new.block 
      format.url output
      format.lastchecked output 
    }
  if$
}

FUNCTION {output.web.refs}
{
  new.block
  output.url
  addeprints eprint empty$ not and
    { format.eprint output.nonnull }
    'skip$
  if$
  adddoiresolver doi empty$ not and
    { format.doi output.nonnull }
    'skip$
  if$
}

% Wrapper for output.bibitem.original.
% If the URL field is not empty, set makeinlinelink to be true,
% so that an inline link will be started at the next opportunity
FUNCTION {output.bibitem}
{ outside.brackets 'bracket.state :=
  output.bibitem.original
  inlinelinks url empty$ not and
    { #1 'makeinlinelink := }
    { #0 'makeinlinelink := }
  if$
}

% Wrapper for fin.entry.original
FUNCTION {fin.entry}
{ output.web.refs  % urlbst
  makeinlinelink       % ooops, it appears we didn't have a title for inlinelink
    { setup.inlinelink % add some artificial link text here, as a fallback
      "[link]" output.nonnull }
    'skip$
  if$
  bracket.state close.brackets = % urlbst
    { "]" * }
    'skip$
  if$
  fin.entry.original
}

% Webpage entry type.
% Title and url fields required;
% author, note, year, month, and lastchecked fields optional
% See references 
%   ISO 690-2 http://www.nlc-bnc.ca/iso/tc46sc9/standard/690-2e.htm
%   http://www.classroom.net/classroom/CitingNetResources.html
%   http://neal.ctstateu.edu/history/cite.html
%   http://www.cas.usf.edu/english/walker/mla.html
% for citation formats for web pages.
FUNCTION {webpage}
{ output.bibitem
  author empty$
    { editor empty$
        'skip$  % author and editor both optional
        { format.editors output.nonnull }
      if$
    }
    { editor empty$
        { format.authors output.nonnull }
        { "can't use both author and editor fields in " cite$ * warning$ }
      if$
    }
  if$
  new.block
  title empty$ 'skip$ 'setup.inlinelink if$
  format.title "title" output.check
  inbrackets "online" output
  new.block
  year empty$
    'skip$
    { format.date "year" output.check }
  if$
  % We don't need to output the URL details ('lastchecked' and 'url'),
  % because fin.entry does that for us, using output.web.refs.  The only
  % reason we would want to put them here is if we were to decide that
  % they should go in front of the rather miscellaneous information in 'note'.
  new.block
  note output
  fin.entry
}
EOD

    print OUT "$mymarkerend\n\n\n";
}


sub print_missing_functions {
    # We've got to the bit of the file which handles the entry
    # types, so write out the webpage entry handler.  This uses
    # the format.date function, which which many but not all
    # bst files have (for example, apalike doesn't).  So
    # check that we either have found this function already, or
    # add it.
    if (! $found{formatdate}) {
	if ($found{entrymonth}) {
	    print OUT <<'EOD';
FUNCTION {format.date}
{ year empty$
    { month empty$
	{ "" }
	{ "there's a month but no year in " cite$ * warning$
	  month
	}
      if$
    }
    { month empty$
	'year
	{ month " " * year * }
      if$
    }
  if$
}
EOD
	} else {
	    print OUT <<'EOD';
FUNCTION {format.date}
{ year empty$
    'skip$
    { %write$
      "(" year * ")" *
    }
  if$
}
EOD
  	}
	$found{formatdate} = 1;
    }

    # If the style file didn't supply a format.title function, then supply
    # one here (the {webpage} function requires it).
    if (! $found{formattitle}) {
	print OUT <<'EOD';
FUNCTION {format.title}
{ title empty$
    { "" }
    { title "t" change.case$ }
  if$
}
EOD
    $found{formattitle} = 1;
    }
}

# Utility function: Keep track of open and close braces in the string argument.
# Keep state in $bracematchtotal, return the current value.
sub bracematcher {
    my $s = shift;
    $s =~ s/[^\{\}]//g;
    #print "s=$s\n";
    foreach my $c (split (//, $s)) {
	$bracematchtotal += ($c eq '{' ? 1 : -1);
    }
    return $bracematchtotal;
}

# Utility function: use bracematcher to copy the complete block which starts
# on or after the current line.
sub copy_block {
    $bracematchtotal = 0;
    # copy any leading lines which don't have braces (presumably comments)
    while (defined ($line = <IN>) && ($line !~ /{/)) {
        print OUT $line;
    }
    while (defined ($line) && bracematcher($line) > 0) {
        print OUT $line;
        $line = <IN>;
    }
    print OUT "$line\n";	# print out terminating \} (assumed
    				# alone on the line)
}

